Occupancy Information Ratio: Infinite-Horizon, Information-Directed, Parameterized Policy Search

In this work, we propose an information-directed objective for infinite-horizon reinforcement learning (RL), called the occupancy information ratio (OIR), inspired by the information ratio objectives used in previous information-directed sampling schemes for multi-armed bandits and Markov decision processes as well as recent advances in general utility RL. The OIR, comprised of a ratio between the average cost of a policy and the entropy of its induced state occupancy measure, enjoys rich underlying structure and presents an objective to which scalable, model-free policy search methods naturally apply. Specifically, we show by leveraging connections between quasiconcave optimization and the linear programming theory for Markov decision processes that the OIR problem can be transformed and solved via concave programming methods when the underlying model is known. Since model knowledge is typically lacking in practice, we lay the foundations for model-free OIR policy search methods by establishing a corresponding policy gradient theorem. Building on this result, we subsequently derive REINFORCE- and actor-critic-style algorithms for solving the OIR problem in policy parameter space. Crucially, exploiting the powerful hidden quasiconcavity property implied by the concave programming transformation of the OIR problem, we establish finite-time convergence of the REINFORCE-style scheme to global optimality and asymptotic convergence of the actor-critic-style scheme to (near) global optimality under suitable conditions. Finally, we experimentally illustrate the utility of OIR-based methods over vanilla methods in sparse-reward settings, supporting the OIR as an alternative to existing RL objectives.

==> sections/Broadening_Horizons.tex <==
\section{Broadening the Information Ratio's Horizons} \label{sec:horizons}

Our goal in this paper is to develop policy search methods for optimizing the rate of exploitation per unit exploration in the infinite-horizon RL setting that are scalable to large state and action spaces through suitable use of policy and value function parameterization. We propose to do this by minimizing the OIR defined in \eqref{eqn:OIR}. As discussed in the related works section, however, information ratios that capture a certain notion of exploitation per unit exploration have already been proposed. It is therefore natural to ask why a new type of information ratio is necessary; cannot policy search methods be developed for optimizing existing information ratios? To answer this question, in this section we review existing information ratio definitions from the multi-armed bandit and recent RL literatures. We then examine the difficulties that arise when trying to formulate policy search schemes for these information ratios. Finally, we explain why the OIR objective is better-suited for policy search in infinite-horizon RL, and how it exhibits better scaling with respect to the cardinality of the state and action~spaces.

\subsection{Existing Information Ratios}

We now present the information ratios developed in the previous works \cite{russo2014learning, russo2016information} and \cite{lu2021reinforcement}. This will allow us to highlight the key differences from the OIR in the following section.
\\ \\
\noindent \textbf{Multi-Armed Bandits.} We first discuss the information ratio considered in \cite{russo2014learning, russo2016information}. Let a finite set of actions $\mathcal{A}$, a set $\mathcal{Y}$ of outcomes, and a reward function $R : \mathcal{Y} \rightarrow \mathbb{R}$ be given. In the multi-armed bandit (MAB) problem, at timestep $t \in \mathbb{N}$, the agent chooses action $a_t \in \mathcal{A}$, observes outcome $Y_{t, a} \in \mathcal{Y}$, and receives reward $R_{t, a} = R(Y_{t, a})$. Let $Y_t = [Y_{t, a}]_{a \in \mathcal{A}}$ denote the vector of possible outcomes at time $t$, and assume there exists a random variable $Z$ such that the sequence of random variables $\{ Y_t \ | \ Z \}_{t \in \mathbb{N}}$ conditioned on $Z$ is i.i.d. Given $Z$, denote the optimal (or an optimal, in the case of multiple optima) action by $A^* \in \argmax_a \mathbb{E} [ R_{1, a} \ | \ Z ]$.

Let $\mathcal{F}_t = \sigma(A_1, Y_{1, A_1}, \ldots, A_{t-1}, Y_{t-1, A_{t-1}})$ denote the $\sigma$-algebra generated by the trajectory up to time $t$. Define a policy $\pi = \{ \pi_t \}_{t \in \mathbb{N}}$ as a sequence of mappings $\pi_t : \mathcal{F}_t \rightarrow \mc{D}(\mathcal{A})$ from trajectories to distributions over the action set. Furthermore, let $\alpha_t(a) = P(A^* = a \ | \ \mathcal{F}_t)$ denote the posterior distribution of $A^*$ given $\mathcal{F}_t$. Define the instantaneous expected regret of choosing a given action at timestep $t$ to be
%
$$\Delta_t(a) = \mathbb{E} \left[ R_{t, A^*} - R_{t, a} \ | \ \mathcal{F}_t \right].$$
%

Given two discrete random variables $X$ and $Y$ defined on the same probability space, the {\em mutual information} $I(X; Y)$ between $X$ and $Y$ is defined in \cite{gray2011entropy} to be
%
$$I(X; Y) = D_{KL} \left[ P_{X, Y} \ || \ P_X \times P_Y \right] = \sum_u \log \left( \frac{P_{X, Y}(u)}{P_X(u) P_Y(u)} \right) P_{X, Y}(u),$$
%
the Kullback-Leibler divergence between the joint distribution of $X, Y$ and the product of their marginals. The mutual information has the following property:
%
\begin{align*}
    I(X; Y) &= H(X) + H(Y) - H(X, Y) \\
    &= H(X) - H(X \ | \ Y) = H(Y) - H(Y \ | \ X),
\end{align*}
%
where $H(X) = - \sum_x \log(p_X(x)) p_X(x)$ and $H(X \ | \ Y) = - \sum_y p_Y(y) \sum_x \log(p_{X|Y}(x \ | \ y)) p_{X|Y}(x \ | \ y)$. The conditional mutual information of random variables $X, Y$ conditioned on $\mathcal{F}_t$, called the {\em mutual information under the posterior distribution} in \cite{russo2014learning}, is given by
%
\begin{equation*}
    I_t(X; Y) = D_{KL} \left[ P((X, Y) \in \cdot \ | \ \mathcal{F}_t ) \ || \ P(X \in \cdot \ | \ \mathcal{F}_t) \times P(Y \in \cdot \ | \ \mathcal{F}_t) \right]
\end{equation*}

The {\em information gain} at time $t$ of action $a$ is defined in \cite{russo2014learning} to be $g_t(a) = I_t ( A^*; Y_{t, a})$ and satisfies the equality
%
\begin{equation*}
    g_t(a) = I_t ( A^*; Y_{t, a}) = \mathbb{E} \left[ H(\alpha_t) - H(\alpha_{t+1}) \ | \ \mathcal{F}_t \right],
\end{equation*}
%
which can be understood as the reduction in uncertainty in the posterior over the optimal action. Finally, given an action sampling distribution $\pi \in \mathcal{D}(\mathcal{A})$, the expected instantaneous regret and information gain are given by $\Delta_t(\pi) = \sum_a \pi(a) \Delta_t(a)$ and $g_t(\pi) = \sum_a \pi(a) g_t(a)$, respectively.
\\ \\
\noindent \textbf{Information Ratio for MABs.} At time $t$, then, the information ratio of an action sampling distribution $\pi$ is defined as \cite{russo2014learning}
%
\begin{equation} \label{eqn:MAB_info_ratio}
    \Psi_t(\pi) = \frac{[\Delta_t(\pi)]^2}{g_t(\pi)},
\end{equation}
%
providing a useful quantity relating the squared instantaneous regret to the information gained about the optimal action by following policy $\pi$.
In addition to its use as an analysis tool for obtaining improved regret bounds \cite{russo2016information}, the information ratio \eqref{eqn:MAB_info_ratio} is used to guide exploration using the information-directed sampling scheme presented in \cite{russo2014learning} for optimizing bandit problems. This amounts to finding and sampling according to a $\pi$ minimizing \eqref{eqn:MAB_info_ratio} at each timestep. This objective balances minimizing regret in the numerator with maximizing the information gained about the optimal action in the denominator. Note that, unlike the infinite-horizon objective \eqref{eqn:OIR}, the numerator and denominator in \eqref{eqn:MAB_info_ratio} are both finite-horizon, single-timestep quantities.
%
\\ \\
\noindent \textbf{General Sequential Decision-Making Problems.} We now turn to the general information ratio defined in \cite{lu2021reinforcement}. Consider an environment given by $\mc{E} = (\mc{A}, \mc{O}, p)$, where $\mc{A}$ is a finite action set, $\mc{O}$ is a finite observation set, and the transition function $p : \mc{H} \times \mc{A} \rightarrow \mc{D}(\mc{O})$ gives a probability distribution $p(\cdot | h, a)$ over $\mc{O}$ for each history-action pair $(h, a) \in \mc{H} \times \mc{A}$, where $\mc{H}$ is the set of all possible state-observation trajectories, i.e. $\mc{H} = \{ (a_0, o_0, a_1, o_1, \ldots, a_t, o_t) \ | \ t \in \mathbb{N}\}$. Furthermore, let a reward function $r : \mc{H} \times \mc{A} \times \mc{O} \rightarrow \mathbb{R}$ be given. In this general setting, at timestep $t \in \{0, \ldots, T-1\}$, for some integer $T$, and equipped with policy $\pi : \mc{H} \rightarrow \mc{D}(\mc{A})$, the agent observes the current history $h_t$, selects an action $a_t \sim \pi(\cdot | h_t)$, sees observation $o_{t+1}$, receives reward $r_t = r(h_t, a_t, o_{t+1})$, and finally sets $t \gets t+1$ and repeats until $t = T$. Note that this general formulation contains MDPs as a special case.

Given a policy $\pi$ and history $h$, let $V_{\pi}(h) = \mathbb{E}_{\pi} \left[ \sum_{t=|h|}^{T-1} r_t \ | \ h \right]$ denote the expected total reward of following policy $\pi$ starting from history $h$ onward, where $|h|$ denotes the time index of the last element of the trajectory $h$. Similarly, let $Q_{\pi}(h, a) = \mathbb{E}_{\pi} \left[ \sum_{t=|h|}^{T-1} r_t \ | \ h, a \right]$ denote the expected total reward of taking action $a$ at history $h$, then afterwards following policy $\pi$. Furthermore, let $V_*(h) = \sup_{\pi} V_{\pi}(h)$ and $Q_*(h, a) = \sup_{\pi} Q_{\pi}(h, a)$ denote the optimal value and action-value functions, respectively. Using these, the expected immediate shortfall is defined as $\mathbb{E}_{\pi} \left[ V_* (h_t) - Q_* (h_t, a_t) \right]$. For the precise definitions of all of these quantities, see \cite{lu2021reinforcement}.

%%% USE THIS IF THE MAB SECTION IS REMOVED
% Given two discrete random variables $X$ and $Y$ defined on the same probability space, the mutual information between $X$ and $Y$ is defined in \cite{gray2011entropy} to be $\mathbb{I}(X; Y) = D_{KL} \left[ P_{X, Y} \ || \ P_X \times P_Y \right] = \sum_u \log \left( \frac{P_{X, Y}(u)}{P_X(u) P_Y(u)} \right) P_{X, Y}(u)$, the Kullback-Leibler divergence between the joint distribution of $X, Y$ and the product of their marginals. Given a third random variable $Z$, the conditional mutual information of random variables $X, Y$ conditioned on $Z$ is given by
% %
% \begin{equation*}
%     \mathbb{I}(X; Y | Z) = D_{KL} \left[ P((X, Y) \in \cdot \ | \ Z ) \ || \ P(X \in \cdot \ | \ Z) \times P(Y \in \cdot \ | \ Z ) \right].
% \end{equation*}

Next, let the random variable $\chi$ denote the abstract learning target of the agent, representing its goals while exploring the environment $\mc{E}$. Furthermore, let $P_t$ denote the agent's learned, finite representation of $\mc{E}$ at time $t$, called the \textit{epistemic state} of the agent. This can include parameters of any learned models of the environment, such as value function approximators or policies. Notice that, conditional on $P_t$, $\mc{E}$ can be viewed as a random variable from the agent's perspective. Recalling the definition of conditional mutual information from above, $\mathbb{I}(\chi; \mc{E} | P_t)$ can be understood as the mutual information between the learning target $\chi$ and environment $\mc{E}$ given the agent's current epistemic state $P_t$. Given a number of timesteps $\tau$, the quantity $\mathbb{I}(\chi; \mc{E} | P_t) - \mathbb{I}(\chi; \mc{E} | P_{t+\tau})$ thus represents the total reduction in uncertainty about the learning target between timesteps $t$ and $t + \tau$. Again, for precise definitions and a thorough discussion, we refer the reader to \cite{lu2021reinforcement}.
%
\\ \\
%
\noindent \textbf{General $\tau$-Information Ratio.} With the foregoing in mind, the $\tau$-information ratio from time $t$ to time $t + \tau$ is defined as
%
\begin{equation} \label{eqn:general_info_ratio}
    \Gamma_{\tau, t} = \frac{\mathbb{E} \left[ V_* (h_t) - Q_* (h_t, a_t) \right]^2}{ \left[ \mathbb{I}(\chi; \mc{E} | P_t) - \mathbb{I}(\chi; \mc{E} | P_{t+\tau}) \right] / \tau },
\end{equation}
%
where the expectation in the numerator is taken with respect to the agent's policy at time $t$. When starting with a policy $\pi$ at time $t$, this quantity has an intuitive interpretation as the ratio of the squared immediate shortfall to the average information gained about the learning target $\chi$ over the subsequent $\tau$ timesteps. Similar to \eqref{eqn:MAB_info_ratio} for the MAB setting, the $\tau$-information ratio is useful as a theoretical tool for obtaining regret bounds. Though the authors recognize that directly optimizing \eqref{eqn:general_info_ratio} is difficult in general, they propose optimizing various proxies, ultimately proposing variants of Q-learning with exploration strategies based on minimizing the $\tau$-information ratio. However, without any parameterization of the the reduction in mutual information betweeen the epistemic state and the learning target of the agent, optimizing this quantity is intractable for large spaces. Moreover, like its predecessor \eqref{eqn:MAB_info_ratio}, and unlike \eqref{eqn:OIR}, the ratio \eqref{eqn:general_info_ratio} is a decidedly finite-horizon objective. We will have more to say about this in the following section.


\subsection{Why the \textit{Occupancy} Information Ratio?}

We next outline the difficulties in applying policy search to the information ratio \eqref{eqn:general_info_ratio} developed in \cite{lu2021reinforcement} and discuss why our OIR objective \eqref{eqn:OIR} is better-suited for policy search algorithms in the infinite-horizon RL setting.

In this paper we focus on developing policy search methods that optimize exploitation per unit exploration. We focus in particular on the infinite-horizon setting, which is the de facto standard in the policy gradient literature and enjoys well-developed underlying theory. Though we consider finite $\mc{S}$ and $\mc{A}$ for the purposes of analysis, an additional goal of this work is to lay the foundations for future development of practical methods that scale to continuous spaces; the success of policy search methods in such settings \cite{schulman2015trust, schulman2017proximal, haarnoja2018soft} motivates our focus on policy search. At the same time, since we are interested in optimizing exploitation per unit exploration, we naturally look to the information ratio work \cite{russo2014learning} and especially \cite{lu2021reinforcement} for inspiration.
%
% Given our focus on policy search for the infinite-horizon setting with an eye towards extensibility to continuous spaces; however, attempting to directly optimize the information ratio \eqref{eqn:general_info_ratio} proposed in \cite{lu2021reinforcement} with respect to the parameters of some policy class is not practicable for two main reasons:
%
However, attempting to perform infinite-horizon policy search using the information ratio \eqref{eqn:general_info_ratio} proposed in \cite{lu2021reinforcement} directly is not practicable for two main reasons:
%
first, the $\tau$-information ratio \eqref{eqn:general_info_ratio} is fundamentally tied to the finite-horizon setting; second, the proxies for \eqref{eqn:general_info_ratio} suggested in \cite{lu2021reinforcement} are only tractable in the finite action space case. This motivates our development of the OIR as a surrogate for optimizing exploitation per unit exploration, since it is well-suited to policy gradient methods and leads to algorithms with robust convergence theory.

To see why the $\tau$-information ratio \eqref{eqn:general_info_ratio} is fundamentally tied to the finite-horizon setting, note that the value and action-value functions $V_*$ and $Q_*$ in the numerator are defined with respect to a fixed horizon $T$, while the epistemic states $P_t$ and $P_{t + \tau}$ are separated by a fixed, finite interval $\tau$. This dependence on $T$ makes development of scalable policy search difficult, as existing policy gradient techniques are overwhelmingly for the infinite-horizon case. Even if dependence of the numerator of \eqref{eqn:general_info_ratio} on $T$ can be removed, the problem still remains of how to deal with the finite $\tau$ in the denominator. A simple idea is to take $\tau \rightarrow \infty$ and consider $\lim_{\tau \rightarrow \infty} \mathbb{I}(\chi; \mc{E} | P_{t + \tau})$, but this leaves us with two problems: first, how do we interpret conditioning mutual information on an infinite trajectory? Second, given the difficulty of estimating mutual information conditioned on a finite trajectory, how can we estimate it when conditioned on an infinite one? It is unclear whether these questions have satisfactory answers.

Nonetheless, while developing the value-IDS and variance-IDS schemes [cf. Sec. \ref{sec:related_work}], \cite{lu2021reinforcement} proposes several proxy ratios for \eqref{eqn:general_info_ratio}. Though these proxies are important and useful guides for short-term exploration, all are still firmly planted in the finite-horizon setting, without clear infinite-horizon analogues. Furthermore, assuming the issues of numerically estimating conditional mutual information and other hard-to-approximate quantities can be resolved, the use of these proxies still involves minimizing over the space $\mc{D}(\mc{A})$ of probability distributions over the action space. This intrinsically links these proxy versions of \eqref{eqn:general_info_ratio} to the finite action space case, which runs counter to our goal of developing an information ratio-inspired policy search scheme that can eventually scale to continuous spaces.

For these reasons, we propose the OIR defined in \eqref{eqn:OIR} as a surrogate for optimizing exploitation per unit exploration via policy search in the infinite-horizon setting. The OIR enjoys several attractive qualities. First, it has a natural interpretation as expected cost per unit information gained about the environment, providing an intuitive measure of the rate of exploitation per unit exploration of a given policy. Second, due to the entropy gradient theorem proved below, the gradient of \eqref{eqn:OIR} can be easily estimated, enabling development of variants of classic policy gradient schemes, such as REINFORCE \cite{williams1992simple} and actor-critic \cite{konda02, bhatnagar2009natural}, in parameterized settings that exhibit tractable scaling to large spaces. In particular, due to the ease with which our framework admits the use of neural network function approximators, OIR variants of modern deep learning-based policy optimization schemes \cite{schulman2015trust, schulman2017proximal} are possible. Finally, methods based on the OIR enjoy robust underlying theory and strong convergence guarantees, as well as promising empirical performance.

==> sections/Experiments_Main_Body.tex <==
\section{Experiments} \label{sec:experiments_main_body}



%
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{images/gridworld2_2_comparison.png}
%     % \captionsetup{width=0.6\linewidth}
%     \captionof{figure}{Comparison of tabular, softmax policy versions of vanilla actor-critic and IDAC with $\kappa = 1.0$ on \texttt{GridWorld2}. Optimal average cost is 1.
%     %
%     Cost: both algorithms decrease to 10; vanilla AC gets stuck, IDAC's cost decreases well below 10.
%     %
%     Entropy: vanilla AC's policy becomes deterministic, while IDAC maintains higher-entropy policies.
%     %
%     OIR: IDAC minimizes the OIR, vanilla AC increases it.
%     }
%     \label{fig:gridworld2}
% \end{figure*}
%
% As discussed in the introduction, OIR methods balance minimizing cost with maintaining a healthy skepticism about their environment. This keeps the agent vigilant against potential \textit{black swan} events -- low-probability events that can have powerful and destabilizing impacts \cite{taleb2007black}. Imagine a turkey destined to be cooked for its farmer's Thanksgiving Day meal \cite{taleb2007black}. Based on its experience being cared-for by the farmer, the turkey's confidence in its safety and well-being grows. The day before Thanksgiving, when the risk to its life is highest, the turkey's confidence is ironically also highest. Instead of trying to escape, the turkey experiences a lethal black swan event and is eaten for Thanksgiving. Casting the turkey's trajectory in reinforcement learning terms, it prematurely converged to a spurious, suboptimal policy by placing too much faith in its insufficiently informative past experience.
%
% \begin{wrapfigure}{r}{0.5\textwidth}
% % \begin{figure}[ht]
% \vspace{-0.5cm}
% \begin{center}
% \centerline{\includegraphics[width=0.5\textwidth]{images/sb3_comparison.png}}
% \caption{Comparison of neural network IDAC with common deep RL methods on the sparse-reward \texttt{LargeGridWorld}. Plots give means and 95\% confidence intervals. Optimal average cost is 0.1. Training took place over $1\mathrm{e}{+6}$ timesteps; no further improvement occurred beyond timestep $1.2\mathrm{e}{+5}$.}
% \label{fig:large_gridworld}
% \end{center}
% \vspace{-0.5cm}
% % \end{figure}
% \end{wrapfigure}

The experiments presented in this section demonstrate that OIR policy gradient methods avoid spurious behavior, while state-of-the-art methods can become overconfident and settle into suboptimality. In particular, when the reward signal is sparse, OIR methods can lead to improved performance when compared with vanilla RL methods. For Fig. \ref{fig:large_gridworld}, we first compared a neural network version of IDAC with the Stable Baselines 3 implementations \cite{raffin2019stable} environment depicted in Fig. \ref{fig:gridworlds}; for Fig. \ref{fig:gridworld2}, we also compared tabular versions of IDAC and vanilla actor-critic with softmax policies on the \texttt{GridWorld2} depicted in Fig. \ref{fig:gridworlds}. Details on the gridworlds are provided in Appendix \ref{sec:experiments}.
%
In all cases, the vanilla methods prematurely converge to suboptimal policies, whereas the OIR-based methods solve the problem. This illustrates that, in sparse-reward environments, the inherent skepticism of OIR-based policy gradient methods can lead to improved performance over current baselines.
Additional experiments illustrating improved performance and validating the theoretical results of \S\S\ref{sec:elements_of_OIR}-\ref{sec:theoretical_results} are provided in Appendix \ref{sec:experiments}.

==> sections/OIR_Pseudocode.tex <==
\section{Algorithms for OIR Minimization}

\begin{algorithm}[H] % enter the algorithm environment
\caption{ID-REINFORCE} % give the algorithm a caption
\label{alg:InfoREINFORCE} % and a label for \ref{} commands later in the document
%\begin{minipage}[!t]{0.49\textwidth}
\begin{algorithmic}[1] % enter the algorithmic environment
\STATE{{\textbf{Initialization:}} Select rollout length $K$, step-sizes $\eta > 0$ and $\tau \in (0, 1]$, parametrized policy class $\{ \pi_{\theta} \}_{\theta \in \Theta}$, and entropy additive constant $\kappa \geq 0$. Randomly sample $s_0$ and $\theta_0$, select $\mu^H_{-1}$, $\mu^J_{-1} > 0$, and set $t \gets 0$.}
\REPEAT
    \STATE Generate trajectory $\{ (s_i, a_i) \}_{i = 1, \ldots, K}$ using $\pi_{\theta_t}$
    %
    \STATE $\widehat{J(\theta_t)} = \frac{1}{K} \sum_{i=1}^{K} c(s_i, a_i)$
    %
    \STATE $\mu^J_t = (1 - \tau) \mu^J_{t-1} + \tau \widehat{J(\theta_t)}$ % \Comment*[r]{Update $J(\theta)$ estimate} % \\
    %
    % Compute estimate $\widehat{\nabla J(\theta_t)} = \frac{1}{K} \sum_{i=1}^K \left[ c(s_i, a_i) - \widetilde{\mu}^J_t \right] \nabla \log \pi_{\theta_t}(a_i | s_i)$ \\
    %
    % Compute estimate $\widehat{d_{\theta_t}}(s_i)$, for each $i = 1, \ldots, K$ \\
    %
    \STATE $d_{\theta_t} = \textsc{DensityEstimator}(\theta_t)$ % \Comment*[r]{Call to oracle} % \\
    %
    \STATE $\widehat{H(d_{\theta_t})} = \frac{1}{K} \sum_{i=1}^K \left(- \log d_{\theta_t}(s_i) \right)$
    %
    \STATE $\mu^H_t = (1 - \tau) \mu^H_{t-1} + \tau \widehat{H(d_{\theta_t})}$ % \Comment*[r]{Update $H(d_{\theta})$ estimate} % \\
    %
    %
    % \small
    % \STATE $\widehat{\nabla \rho(\theta_t)} = \frac{1}{\left[ \kappa + \widetilde{\mu}^H_t \right]^2} \frac{1}{K} \sum_{i=1}^K \left[ \left( c(s_i, a_i) - \widetilde{\mu}^J_t \right) \left(\kappa + \widetilde{\mu}^H_t \right)  - \widetilde{\mu}^J_t \left( - \log d_{\theta_t}(s_i) - \widetilde{\mu}^H_t \right) \right] \nabla \log \pi_{\theta_t}(a_i | s_i)$
    % \normalsize
    %
    \FOR{$i = 1, \ldots, k$}
        \STATE $\delta_i^J = c(s_i, a_i) - \mu^J_t$
        %
        \STATE $\delta_i^H = - \log d_{\theta_t}(s_i) - \mu^H_t$
        %
        \STATE $\psi_i = \nabla \log \pi_{\theta_t}(a_i | s_i)$
    \ENDFOR
    %
    \small
    \STATE $\widehat{\nabla \rho(\theta_t)} = \frac{1}{\left[ \kappa + \mu^H_t \right]^2} \frac{1}{K} \sum_{i=1}^K \left[ \delta_i^J \left(\kappa + \mu^H_t \right)  - \mu^J_t \delta_i^H \right] \psi_i$
    \normalsize
    %
    \STATE $\theta_{t+1} = \theta_t - \eta \widehat{\nabla \rho(\theta_t)}$ % \Comment*[r]{Policy gradient update} % \\
    %
    \STATE $t \gets t + 1$
\UNTIL{convergence}
\end{algorithmic}
%\end{minipage}
\end{algorithm}




\begin{algorithm}[H] % enter the algorithm environment
\caption{IDAC} % give the algorithm a caption
\label{alg:irac} % and a label for \ref{} commands later in the document
%\begin{minipage}[!t]{0.49\textwidth}
\begin{algorithmic}[1] % enter the algorithmic environment
\STATE{{\textbf{Initialization:}} Select rollout length $K$, stepsize sequences $\{ \alpha_t \}, \{ \beta_t \}, \{ \tau_t \}$, parametrized policy class $\{ \pi_{\theta} \}_{\theta \in \Theta}$, parametrized critic class $\{ v_{\omega} \}_{\omega \in \Omega}$, and entropy additive constant $\kappa \geq 0$. Randomly sample $s_0, \theta_0, \omega_0^J, \omega_0^H$, select $\mu^H_{-1}$, $\mu^J_{-1} > 0$, and set $t \gets 0$.}
\REPEAT
    \STATE Generate trajectory $\{ (s_i, a_i) \}_{i = 1, \ldots, K}$ using $\pi_{\theta_t}$
    %
    % $\widehat{J(\theta_t)} = \frac{1}{K} \sum_{i=1}^{K} c(s_i, a_i)$ \\
    % %
    % $\widetilde{\mu}^J_t = (1 - \tau) \widetilde{\mu}^J_{t-1} + \tau \widehat{J(\theta_t)}$ \\
    %
    \STATE $\mu^J_t = (1 - \tau) \mu^J_{t-1} + \tau \frac{1}{K} \sum_{i=1}^{K} c(s_i, a_i)$ % \Comment*[r]{Update $J(\theta)$ estimate} % \\
    %
    % Compute estimate $\widehat{d_{\theta_t}}(s_i),$ for each $i = 1, \ldots, K$ \\
    %
    \STATE $d_{\theta_t} = \textsc{DensityEstimator}(\theta_t)$ % \Comment*[r]{Call to oracle} % \\
    %
    % $\widehat{H(d_{\theta_t})} = \frac{1}{K} \sum_{i=1}^K \left(- \log d_{\theta_t}(s_i) \right)$ \\
    % %
    % $\widetilde{\mu}^H_t = (1 - \tau) \widetilde{\mu}^H_{t-1} + \tau \widehat{H(d_{\theta_t})}$ \\
    %
    \STATE $\mu^H_t = (1 - \tau) \mu^H_{t-1} + \tau \frac{1}{K} \sum_{i=1}^K \left(- \log d_{\theta_t}(s_i) \right)$ % \Comment*[r]{Update $H(d_{\theta})$ estimate} % \\
    %
    \FOR{$i = 1, \ldots, K$}
        \STATE Set $v_{\omega^J_t}(s_{K+1}) = v_{\omega^H_t}(s_{K+1}) = 0$
        %
        % Compute TD errors: \\
        \STATE $\delta^J_i = c(s_i, a_i) - \mu^J_t + v_{\omega^J_t}(s_{i+1}) - v_{\omega^J_t}(s_i)$ % \Comment*[r]{Compute cost TD error at $s_i$} % \\
        %
        \STATE $\delta^H_i = - \log d_{\theta_t}(s_i) - \mu^H_t + v_{\omega^H_t}(s_{i+1}) - v_{\omega^H_t}(s_i)$ % \Comment*[r]{Compute entropy TD error at $s_i$} % \\
        %
        \STATE $\psi_i = \nabla \log \pi_{\theta_t}(a_i | s_i)$
        %
        % where we stipulate $v_{\omega^J_t}(s_{K+1}) = v_{\omega^H_t}(s_{K+1}) = 0$
    \ENDFOR
    %
    % $\widehat{\nabla v_{\omega^J_t}} = \frac{1}{K} \sum_{i=1}^K \delta^J_i \nabla v_{\omega^J_t}(s_i)$ \\
    % %
    % $\omega^J_{t+1} = \omega^J_t + \alpha \widehat{\nabla v_{\omega^J_t}}$ \\
    %
    \STATE $\omega^J_{t+1} = \omega^J_t + \alpha \frac{1}{K} \sum_{i=1}^K \delta^J_i \nabla v_{\omega^J_t}(s_i)$  % \Comment*[r]{Cost critic update} % \\
    %
    % $\widehat{\nabla v_{\omega^H_t}} = \frac{1}{K} \sum_{i=1}^K \delta^H_i \nabla v_{\omega^H_t}(s_i)$ \\
    % %
    % $\omega^H_{t+1} = \omega^H_t + \alpha \widehat{\nabla v_{\omega^H_t}}$ \\
    %
    \STATE $\omega^H_{t+1} = \omega^H_t + \alpha \frac{1}{K} \sum_{i=1}^K \delta^H_i \nabla v_{\omega^H_t}(s_i)$ % \Comment*[r]{Entropy critic update} % \\
    %
    \small
    \STATE $\widehat{\nabla \rho(\theta_t)} = \frac{1}{\left[ \kappa + \mu^H_t \right]^2} \frac{1}{K} \sum_{i=1}^K \left[ \delta^J_i \left(\kappa + \mu^H_t \right) - \mu^J_t \delta^H_i \right] \psi_i$
    \normalsize % \Comment*[r]{Policy gradient estimate} % \\
    %
    \STATE $\theta_{t+1} = \theta_t - \beta \widehat{\nabla \rho(\theta_t)}$ % \Comment*[r]{Actor update} % \\
    %
    \STATE $t \gets t + 1$
\UNTIL{convergence}
\end{algorithmic}
%\end{minipage}
\end{algorithm}

==> sections/Proofs_and_Examples.tex <==

\section{Examples} \label{sec:example}


\begin{example} \label{ex:hidden_concavity_example}
Consider an MDP with state space $\mc{S} = \{ s_1, s_2 \}$, action space $\mc{A} = \{ L, R \}$, a transition probability function $p$ satisfying $p(s' | s, a) > 0$, for all $s, s' \in \mc{S}, a \in \mc{A}$, and an arbitrary cost function $c : \mc{S} \times \mc{A} \rightarrow \mathbb{R}$. Given a policy $\pi$, we can represent it in tabular form as a vector $\pi \in \mathbb{R}^4$ with non-negative entries such that $\pi(L | s_i) + \pi(R | s_i) = 1$, for $i \in \{ 1, 2 \}$. The transition probability matrix of the Markov chain induced by $\pi$ on $\mc{S}$ is as follows:
%
\begin{equation*} P_{\pi} =
%
\begin{bmatrix}
    p(s_1 | s_1, L) \pi( L | s_1) + p(s_1 | s_1, R) \pi( R | s_1) & p(s_2 | s_1, L) \pi(L | s_1) + p(s_1 | s_1, R) \pi(R | s_1) \\
    %
    p(s_1 | s_2, L) \pi(L | s_2) + p(s_1 | s_2, R) \pi(R | s_2) & p(s_2 | s_2, L) \pi(L | s_2) | p(s_2 | s_2, R) \pi(R | s_2)
\end{bmatrix}.
\end{equation*}
%
The state occupancy measure $d_{\pi}$ induced by $\pi$ can be obtained by solving the system of equations $P_{\pi}^T d = d, \bm{1}^T d = 1$ in the unknown $d = \begin{bmatrix} d_1 & d_2 \end{bmatrix}^T$. Some simple algebra yields
%
\begin{align*}
    d_1 &= \frac{ p(s_1 | s_2, L) \pi(L | s_2) + p(s_1 | s_2, R) \pi(R | s_2) }{ 1 + p(s_1 | s_2, L) \pi(L | s_2) + p(s_1 | s_2, R) \pi(R | s_2) - p(s_1 | s_1, L) \pi( L | s_1) - p(s_1 | s_1, R) \pi( R | s_1)}.
\end{align*}
%
Notice that, since $p(s_i | s_j, a) > 0, \pi(a | s_i) \geq 0$ and $\pi(L | s_i) + \pi(R | s_i) = 1$, for all $i, j \in \{ 1, 2 \}$ and $a \in \{ L, R \}$, $d_1$ is always defined and strictly positive. Since $d_2 = 1 - d_1$, the same statement holds for $d_2$. The state occupancy measure induced by $\pi$ is thus given by the vector $d_{\pi} = d = \begin{bmatrix} d_1 & d_2 \end{bmatrix}^T$.


%
We now show that, for the MDP $(\mc{S}, \mc{A}, p, c)$ just specified, Assumption \ref{assum:hidden_concavity_info_ratio} holds.
%
Let $\Theta \subset \mathbb{R}^4$ denote the set of vector representations of all valid policies $\pi$, and let $\lambda : \Theta \rightarrow \mc{D}(\mc{S} \times \mc{A})$ denote the function mapping policies $\pi$ to state-action occupancy measures $\lambda(\pi)$. Clearly $\lambda(\pi)(s, a) = d_{\pi}(s) \pi(a | s)$, for all $s \in \mc{S}, a \in \mc{A}$.
%
It is known that part one of Assumption \ref{assum:hidden_concavity_info_ratio} holds (see, e.g., \cite{Puterman_2014}). It can furthermore be shown (see the proof of Prop.~H.2 in \cite{zhang2020variational}) that part two holds. All that remains is to show that part three holds by proving that $\nabla \lambda(\pi)$ is Lipschitz in $\pi$. Notice that the identity function is Lipschitz and trivially bounded over any bounded domain, and recall that the product of two Lipschitz and bounded functions is a Lipschitz function. Since the domain $\Theta$ is bounded, this means that, if $d_{\pi}$ is Lipschitz and bounded in $\pi$, it will follow that $\lambda(\pi)$ is Lipschitz in $\pi$ over $\Theta$, since it is a product of Lipschitz, bounded functions. But the partial derivatives of $d_1$ with respect to $\pi(L | s_1), \pi(R | s_1), \pi(L | s_2),$ and $\pi(R | s_2)$ are all continuous and bounded for all valid policy vectors $\pi$, so $d_1$ is Lipschitz in $\pi$. Since $d_2 = 1 - d_1$, this means that $d_{\pi} = \begin{bmatrix} d_1 & d_2 \end{bmatrix}^T$ is Lipschitz in $\pi$. Finally, we already know that $d_{\pi}$ is bounded, so $\lambda(\pi)$ is therefore Lipschitz in $\pi$, and thus part three of Assumption~\ref{assum:hidden_concavity_info_ratio}~holds.

\end{example}



\section{Proofs and Additional Results} \label{sec:proofs}


\subsection{Proof of Lemma \ref{lemma:entropy_cross_entropy_gradient}}

% \begin{lemma} \label{lemma:entropy_cross_entropy_gradient}
% For any $\theta' \in \Theta$,
% \begin{align} \label{eqn:s_entropy_gradient}
%     \nabla H(d_{\theta}) \big\rvert_{\theta = \theta'} = \nabla CE(d_{\theta}, d_{\theta'}) \big\rvert_{\theta = \theta'}.
% \end{align}
% \end{lemma}
%
\begin{proof}
Notice that
%
\begin{align}
    \nabla CE(d_{\theta}, d_{\theta'}) \big\rvert_{\theta = \theta'} &= \nabla \left[ H(d_{\theta}) + D_{KL}(d_{\theta} \ || \ d_{\theta'}) \right] \big\rvert_{\theta = \theta'} \nonumber \\
    %
    &= \nabla H(d_{\theta}) \big\rvert_{\theta = \theta'} + \nabla D_{KL}(d_{\theta} \ || \ d_{\theta'}) \big\rvert_{\theta = \theta'}. \label{eqn:ce_entropy_kl}
\end{align}
%
Expanding the term $\nabla D_{KL}(d_{\theta} \ || \ d_{\theta'})$, where the gradient is being taken w.r.t. $\theta$ and $\theta'$ is fixed, we get
%
\begin{align*}
    \nabla D_{KL}( d_{\theta} \ || \ d_{\theta'} ) &= \sum_s \nabla \left[ \log \left( \frac{d_{\theta}(s)}{d_{\theta'}(s)} \right) d_{\theta}(s) \right] = \sum_s \nabla \left[ ( \log d_{\theta}(s) - \log d_{\theta'}(s) ) d_{\theta}(s) \right] \nonumber \\
    %
    &\labelrel={eqn:kl1} \sum_s \left[ \left( \nabla [ \log d_{\theta}(s) - \log d_{\theta'}(s) ] \right) d_{\theta}(s) + [ \log d_{\theta}(s) - \log d_{\theta'}(s) ] \nabla d_{\theta}(s) \right] \nonumber \\
    %
    &\labelrel={eqn:kl2} \sum_s \left[ \frac{\nabla d_{\theta}(s)}{d_{\theta}(s)} d_{\theta}(s) + [ \log d_{\theta}(s) - \log d_{\theta'}(s) ] \nabla d_{\theta}(s) \right] \nonumber \\
    %
    &\labelrel={eqn:kl3} \sum_s \left[ 1 + \log d_{\theta}(s) - \log d_{\theta'}(s) \right] \nabla d_{\theta}(s) \;, 
\end{align*}
%
where \eqref{eqn:kl1} follows from the product rule, \eqref{eqn:kl2} holds because $\nabla \log d_{\theta}(s) = [\nabla d_{\theta}(s)] / d_{\theta}(s)$, and the $d_{\theta}(s)$ terms cancel to yield \eqref{eqn:kl3}. Evaluating the last expression at $\theta = \theta'$, we end up with
%
\begin{align*}
    \nabla D_{KL}(d_{\theta} \ || \ d_{\theta'}) \big\rvert_{\theta = \theta'} &= \left( \sum_s \left[ 1 + \log d_{\theta}(s) - \log d_{\theta'}(s) \right] \nabla d_{\theta}(s) \right) \Bigg\rvert_{\theta = \theta'} \\
    %
    &\labelrel={eqn:kl4} \sum_s \left[ 1 + \log d_{\theta'}(s) - \log d_{\theta'}(s) \right] \left( \nabla d_{\theta}(s) \big\rvert_{\theta = \theta'} \right) \\
    %
    &= \sum_s \left( \nabla d_{\theta}(s) \big\rvert_{\theta = \theta'} \right)
    %
    \labelrel={eqn:kl5} \left( \sum_s \nabla d_{\theta}(s) \right) \Bigg\rvert_{\theta = \theta'}
    %
    \labelrel={eqn:kl6} \left( \nabla \sum_s d_{\theta}(s) \right) \Bigg\rvert_{\theta = \theta'} \\
    %
    &\labelrel={eqn:kl7} \nabla 1 \big\rvert_{\theta = \theta'} = 0,
\end{align*}
%
where we evaluate the terms $\log d_{\theta}(s)$ and $\nabla d_{\theta}(s)$ at $\theta = \theta'$ to get \eqref{eqn:kl4}, move the evaluation $\theta = \theta'$ outside the summation in \eqref{eqn:kl5}, pull the gradient outside the summation to obtain \eqref{eqn:kl6}, and finally recall that $\sum_s d_{\theta}(s) = 1$ to get \eqref{eqn:kl7}.
%
But, recalling equation \eqref{eqn:ce_entropy_kl}, this means that
%
\begin{align*}
    \nabla H(d_{\theta}) \big\rvert_{\theta = \theta'} = \nabla CE(d_{\theta}, d_{\theta'}) \big\rvert_{\theta = \theta'},
\end{align*}
%
completing the proof.
\end{proof}


\subsection{Proof of Theorem \ref{thm:entropy_gradient}}

% \begin{theorem}
% %
% Let an MDP $(\mathcal{S}, \mathcal{A}, p, c)$ and a differentiable parametrized policy class $\{ \pi_{\theta} \}_{\theta \in \Theta}$ be given, and recall the definition \eqref{eqn:s_occ_meas} of the state occupancy measure $d_{\theta}$ induced by each $\pi_{\theta}$ on $\mathcal{S}$. Fix a policy parameter iterate $\theta_t$ at timestep $t$. The gradient $\nabla H(d_{\theta}) \rvert_{\theta = \theta_t}$ [cf. \eqref{eqn:s_entropy_gradient}] with respect to the policy parameters $\theta$ of the state occupancy measure entropy $H(d_{\theta})$ [cf. \eqref{eqn:s_entropy}] evaluated at $\theta = \theta_t$ satisfies
% %
% \label{thm:entropy_gradient}
%     \begin{equation} \label{eqn:entropy_gradient}
%         \nabla H(d_{\theta}) \big\rvert_{\theta = \theta_t} = \mathbb{E}_{\pi_{\theta_t}} \Big[ \left( - \log d_{\theta_t}(s) - H(d_{\theta_t}) \right) \nabla \log \pi_{\theta_t}(a | s) \Big].
%     \end{equation}
% \end{theorem}
%
\begin{proof}
    At a given $t$, consider the average-reward MDP $(\mathcal{S}, \mathcal{A}, p, r_t)$, where $r_t: \mathcal{S} \rightarrow \mathbb{R}^+$ is the purely state-dependent (i.e., action-independent) reward given by $r_t(s) = -\log d_{\theta_t}(s)$. We refer to the MDP $(\mathcal{S}, \mathcal{A}, p, r_t)$ as the \textit{shadow MDP} associated with parameter $\theta_t$. Define
    %
    \begin{equation*}
        \mu^t(\theta) = \lim_{n \rightarrow \infty} \frac{1}{n} \mathbb{E} \left[ \sum_{i=1}^n r_t(s_i) \ | \ \pi_{\theta} \right],
    \end{equation*}
    %
    \begin{equation*}
        Q^t_{\theta}(s, a) = \sum_{n=1}^{\infty} \mathbb{E} \left[ r_t(s_n) - \mu^t(\theta) \ | \ s_0 = s, a_0 = a, \pi_{\theta} \right].
    \end{equation*}
    %
    Here $\mu^t(\theta)$ is the expected long-run average reward of using $\pi_{\theta}$ on the shadow MDP $(\mathcal{S}, \mathcal{A}, p, r_t)$, while $Q^t_{\theta}$ is the corresponding state-action value function. Given a policy $\pi_{\theta}$, 
    %
    \begin{equation}
    CE(d_{\theta}, d_{\theta_t}) = - \sum_s d_{\theta}(s) \log d_{\theta_t}(s) = \sum_s d_{\theta}(s) \ r_t(s) = \sum_s d_{\theta}(s) \sum_a \pi_{\theta}(a | s) \ r_t(s),
    \end{equation}
    %
    where the last equality holds by the fact that $\sum_a \pi_{\theta}(a | s) = 1$, for all $s \in \mathcal{S}$.
    %
    The policy gradient theorem \eqref{eqn:classic_pgt} can thus be used to yield the expression
    %
    \begin{equation} \label{eqn:CE_pgt}
        \nabla CE(d_{\theta}, d_{\theta_t}) = \sum_s d_{\theta}(s) \sum_a Q^t_{\theta}(s, a) \nabla \log \pi_{\theta}(a | s).
    \end{equation}
    %
    Combining expression \eqref{eqn:CE_pgt} with Lemma \ref{lemma:entropy_cross_entropy_gradient} and noticing that $\mu^t(\theta_t) = \sum_s d_{\theta_t}(s) \left( - \log d_{\theta_t}(s) \right) = H(d_{\theta_t})$ yields equation \eqref{eqn:entropy_gradient}.
\end{proof}
%


\subsection{State-action Entropy Gradient Theorem}

Recall the definition of the state-action occupancy measure from \S\ref{sec:problem_formulation}, for any policy $\pi_{\theta}, \theta \in \Theta$:
%
\begin{equation} \label{eqn:sa_occ_meas}
    \lambda_{\theta}(s, a) = \lim_{t \rightarrow \infty} P(s_t = s, a_t = a\ | \ \pi_{\theta})
\end{equation}
%
Define the entropy of the state-action occupancy measure induced by $\pi_{\theta}$ to be
%
\begin{equation} \label{eqn:sa_entropy}
    H(\lambda_{\theta}) = - \sum_s \sum_a \lambda_{\theta}(s, a) \log \lambda_{\theta}(s, a)
    %
    % = - \sum_s d_{\theta}(s) \sum_a \pi_{\theta}(a | s) \left[ \log d_{\theta}(s) + \log \pi_{\theta}(a | s) \right].
\end{equation}
%
\begin{corollary} \label{cor:state_action_entropy_gradient}
Let an MDP $(\mathcal{S}, \mathcal{A}, p, c)$ and a differentiable parametrized policy class $\{ \pi_{\theta} \}_{\theta \in \Theta}$ be given, and let $\lambda_{\theta}$ be as in \eqref{eqn:sa_occ_meas}. Fix a policy parameter iterate $\theta_t$ at timestep $t$. The gradient $\nabla H(\lambda_{\theta}) \rvert_{\theta = \theta_t}$ with respect to the policy parameters $\theta$ of the state-action occupancy measure entropy $H(\lambda_{\theta})$ [cf. \eqref{eqn:sa_entropy}] evaluated at $\theta = \theta_t$ satisfies
%
%
    \begin{equation} \label{eqn:state_action_entropy_gradient}
        \nabla H(\lambda_{\theta}) \big\rvert_{\theta = \theta_t} = \mathbb{E}_{\pi_{\theta_t}} \Big[ \left( - \log d_{\theta_t}(s) - \log \pi_{\theta_t}(a | s) - H(\lambda_{\theta_t}) \right) \nabla \log \pi_{\theta_t}(a | s) \Big].
    \end{equation}
\end{corollary}

\begin{proof}
The statement follows by replacing $r_t(s) = - \log d_{\theta_t}(s)$ with $r_t(s, a) = - \log \lambda_{\theta_t}(s, a) = - \log d_{\theta_t}(s) - \log \pi_{\theta_t}(a | s)$ in the proof of Theorem \ref{thm:entropy_gradient}, redefining $\mu^t(\theta)$ and $Q^t_{\theta}$ accordingly, and noting that
%
$$CE(\lambda_{\theta}, \lambda_{\theta_t}) = - \sum_s \sum_a \lambda_{\theta}(s, a) \log \lambda_{\theta_t}(s, a) = \sum_s d_{\theta}(s) \sum_a \pi_{\theta}(a | s)\left[ - \log d_{\theta_t}(s) - \log \pi_{\theta_t}(a | s) \right].$$
%
An application of \eqref{eqn:classic_pgt} then yields the corresponding analogue of \eqref{eqn:CE_pgt}, which can be combined with a state-action analogue of Lemma \ref{lemma:entropy_cross_entropy_gradient} to yield \eqref{eqn:state_action_entropy_gradient}.
\end{proof}



\subsection{Derivation of Concave Transformation of \eqref{opt:Q0}} \label{sec:concave_transformation}


\subsubsection{Quasiconvexity of \eqref{opt:Q0}}

As a first step on our path to showing how to solve \eqref{opt:Q0} using a concave reformulation, we prove that the quasiconvex optimization problem \eqref{opt:Q0} is feasible and that every local optimal solution to it is a global optimal solution. We will then show that the problem can be equivalently formulated as an intermediate quasiconcave optimization problem. We subsequently show how this quasiconcave program can be transformed into a concave program via the range transformation described in Ch. 7 of \cite{avriel2010generalized}. The latter transformation is our end goal, as the resulting concave program can then be efficiently solved to obtain an optimal solution to \eqref{opt:Q0}.

Let us first formally define quasi-convexity/-concavity. Given a scalar $\alpha$ and function $f : \mathbb{R}^n \rightarrow \mathbb{R}$ defined on a convex set $C \subset \mathbb{R}^n$, define the $\alpha$-superlevel set of $f$ on $C$ to be $U(f, \alpha) = \{ x \in C \ | \ f(x) \geq \alpha \}$ and the $\alpha$-sublevel set of $f$ on $C$ to be $L(f, \alpha) = \{ x \in C \ | \ f(x) \leq \alpha \}$.
%
\begin{definition} \label{def:quasiconvex}
Given $f : \mathbb{R}^n \rightarrow \mathbb{R}$ defined on a convex set $C \subset \mathbb{R}^n$, $f$ is \textit{quasiconvex (resp. quasiconcave)} if $L(f, \alpha)$ (resp. $U(f, \alpha)$) is convex, for each $\alpha \in \mathbb{R}$.
\end{definition}
%
\noindent Now let $\Delta(\mathbb{R}^{|\mathcal{S}| \cdot |\mathcal{A}|})$ denote the unit simplex in $\mathbb{R}^{|\mathcal{S}| \cdot |\mathcal{A}|}$, and let $F$ denote the feasible region of \eqref{opt:Q0}. Clearly $F$ is a convex subset of $\Delta(\mathbb{R}^{|\mc{S}| \cdot |\mc{A}|})$, since it is defined by linear equality and nonnegativity constraints. Note that the numerator of $\rho(\lambda)$, the objective function in \eqref{opt:Q0}, is convex (linear, in fact). Also notice that $\widehat{H}(\lambda) = H(d^{\lambda})$ is concave on $F$, which follows from the facts that the entropy $H(d)$ is concave in $d$, $d^{\lambda}$ is a linear function of $\lambda$, and the composition of a concave function with an affine function is itself concave. This implies that, for any fixed $\kappa \geq 0$, the denominator of $\rho(\lambda)$ is concave and also positive by Assumption \ref{assum:two_nonzero_entries} over all its sublevel subsets of the feasible region. These facts guarantee that \eqref{opt:Q0} is a quasiconvex program with a well-behaved objective function, as formalized in the following Lemma.
%
\begin{lemma} \label{lemma:quasiconvex}
\eqref{opt:Q0} is feasible and has an optimal solution with finite objective function value, and the objective $\rho$ of \eqref{opt:Q0} is strictly quasiconvex on $F$.
\end{lemma}
%
\begin{proof}
The problem is clearly feasible, since any arbitrary policy $\pi$ induces a valid state-action occupancy measure $\lambda^{\pi} \in F$. Since $F$ is bounded as a subset of the unit simplex, and also $J(\lambda) > 0$ and $\kappa + \widehat{H}(\lambda) > 0$ on $F$ by Assumption \ref{assum:two_nonzero_entries}, we have that $\rho$ is bounded on $F$. Furthermore, since $J(\lambda)$ is linear on $F$, $\kappa + \widehat{H}(\lambda)$ is concave on $F$, and $J(\lambda) > 0$ and $\kappa + \widehat{H}(\lambda) > 0$ on all the sublevel sets of $\rho$ on $F$, Prop.~5.20 of \cite{avriel2010generalized} applies to show that $\rho$ is quasiconvex on $F$.
\end{proof}
%
%
%
\noindent Finally, \eqref{opt:Q0} enjoys the following key property, which guarantees that any solution to the concave program described in the next section provides a globally optimal solution to the OIR minimization problem \eqref{eqn:OIR}.
%
\begin{lemma} \label{lemma:local_implies_global}
Every local optimum of \eqref{opt:Q0} is a global optimum.
\end{lemma}
%
\begin{proof}
The assertion follows directly from Prop.~3.3 in \cite{avriel2010generalized}.
\end{proof}


\subsubsection{Transformation to a Concave Program}

Now that we are assured \eqref{opt:Q0} is quasiconvex and has no spurious stationary points, we show it can be reformulated as an equivalent concave program. To do so, we first transform it into an equivalent \textit{quasiconcave} maximization problem by showing that minimizing the objective function $\rho(\lambda)$ of problem \eqref{opt:Q0} is equivalent to maximizing its reciprocal $1 / \rho(\lambda)$. Next, we show that, by using a suitable change of variables first proposed in \cite{schaible1976fractional}, this objective function can be reinterpreted as the perspective transform of a concave function, which is itself concave. Finally, we apply results from \cite{avriel2010generalized} to obtain the desired concave reformulation of \eqref{opt:Q0}. As highlighted at the beginning of this section, the definition of the OIR is critical to this reformulation, as it exploits structural attributes of the family of state-action occupancy measures to enable the transformation from the initial quasiconvex program to the desired concave program.

Define $q(\lambda) := 1 / \rho(\lambda) = (\kappa + \widehat{H}(\lambda)) / J(\lambda)$ and consider the problem
%
\begin{maxi*}
  {\lambda}{q(\lambda)}{}{}
    \addConstraint{\sum_s \sum_a \lambda_{sa}}{= 1}{}  \tag{$Q_1$} \label{opt:Q1}
    \addConstraint{\sum_a \lambda_{sa}}{= \sum_{s'} \sum_a p(s | s', a) \lambda_{s'a},}{\hspace{4mm} \forall s \in \mathcal{S}}
    \addConstraint{\lambda}{\geq 0}{}{}.
\end{maxi*}
%
\noindent Note that the feasible region $F$ of \eqref{opt:Q1} is identical to the feasible region of \eqref{opt:Q0}. We have the following result:
%
\begin{lemma} \label{lemma:Q0_eq_Q1}
Problem \eqref{opt:Q0} is equivalent to \eqref{opt:Q1}.
\end{lemma}
%
\begin{proof}
Assume $\lambda^*$ is optimal for \eqref{opt:Q0}, i.e. $\lambda^* \in F$ and $\rho(\lambda^*) \leq \rho(\lambda)$, for all $\lambda \in F$. By Lemma \ref{lemma:quasiconvex}, there exists $M > 0$ such that $0 < \rho(\lambda^*) \leq \rho(\lambda) < M < \infty$, for all $\lambda \in F$. Clearly $0 < 1/M < q(\lambda) \leq q(\lambda^*) < \infty$, for all $\lambda \in F$, so $\lambda^*$ is optimal to \eqref{opt:Q1}. By an analogous argument, any optimal solution to \eqref{opt:Q1} is optimal to~\eqref{opt:Q0}.
%
\end{proof}
%
% \subsubsection{Transformation to a Concave Program}
%
\noindent The foregoing Lemma proves that solving \eqref{opt:Q1} also solves \eqref{opt:Q0}. Crucially, we can in fact transform \eqref{opt:Q1} into a \textit{concave} optimization problem, which will allow us to indirectly solve \eqref{opt:Q0}. Using the variable transformation
%
$$y = \frac{\lambda}{c^T \lambda}, \hspace{2mm} t = \frac{1}{c^T \lambda},$$
%
and applying the key result Prop.~7.2 in \cite{avriel2010generalized}, we obtain the equivalent problem
%
\begin{maxi*}
    {y, t}{t \left[ \kappa + \widehat{H} \left( \frac{y}{t} \right) \right] =
        t \left[ \kappa - \sum_s \left( \frac{\sum_a y_{sa}}{t} \right) \log \left( \frac{ \sum_a y_{sa}}{t} \right) \right]}{}{}
    \addConstraint{t \left[ \sum_s \sum_a \frac{y_{sa}}{t} - 1 \right]}{= 0} \tag{$Q_2$} \label{opt:Q2}
    \addConstraint{t \left[ \sum_a \frac{y_{sa}}{t} - \sum_{s'} \sum_a p(s | s', a) \frac{y_{s'a}}{t} \right]}{= 0,}{\hspace{4mm} \forall s \in \mathcal{S}}
    \addConstraint{t \left[ \sum_s \sum_a c_{sa} \frac{y_{sa}}{t} \right]}{= 1}
    \addConstraint{y \geq 0, \frac{y}{t}}{\geq 0}.
    % \addConstraint{y / t}{\geq 0}.
\end{maxi*}
%
% Proofs that generalized forms of problems \eqref{opt:Q1} and \eqref{opt:Q2} are equivalent can be found in \cite{avriel2010generalized}.
Notice that the constraint $\sum_s \sum_a c_{sa} y_{sa} = 1$, combined with the fact that $c > 0$, implies that $y_{sa} > 0$ for at least one $y_{sa}$. Since $y \geq 0$ and $\sum_s \sum_a y_{sa} = t$, this means $t > 0$. The constraint $y / t \geq 0$ is thus redundant, so it can be removed. The objective and the first two constraints in problem \eqref{opt:Q2} can also be simplified to obtain the following, cleaner form:
%
\begin{maxi*}
    {y, t}{\kappa t - \sum_s \sum_a y_{sa} \log \left( \frac{\sum_a y_{sa}}{t} \right)}{}{}
    \addConstraint{\sum_s \sum_a y_{sa}}{= t} \tag{$Q'$} \label{opt:Q3}
    \addConstraint{\sum_a y_{sa}}{= \sum_{s'} \sum_a p(s | s', a) y_{s'a},}{\hspace{4mm} \forall s \in \mathcal{S}}
    \addConstraint{\sum_s \sum_a c_{sa} y_{sa}}{= 1}
    \addConstraint{y}{\geq 0}.
    % \addConstraint{y / t}{\geq 0}.
\end{maxi*}
%
The constraints clearly define a convex feasible region, and the objective function is also concave, as it is the \textit{perspective} of the function $\kappa + \widehat{H}(\lambda)$, which is defined for the general setting as follows:
%
\begin{definition} \label{def:perspective_transform}
Given $f : \mathbb{R}^n \rightarrow \mathbb{R}$, the \textit{perspective} of $f$ is the function $P_f : \mathbb{R}^{n+1} \rightarrow \mathbb{R}$ given by $P_f(x, t) = t f(x / t)$ with domain $\textbf{dom}(P_f) = \{ (x, t) \ | \ x / t \in \textbf{dom}(f), t > 0\}$.
\end{definition}
%
\noindent As discussed in \S3.6.2 of \cite{boyd2004convex}, the perspective operation preserves concavity/convexity. In particular, if $f$ is concave (resp. convex), then $g$ is concave (resp. convex). Thus \eqref{opt:Q3} is a concave program. Finally, given an optimal solution $(y^*, t^*)$ to \eqref{opt:Q3}, we can recover an optimal solution $\lambda^* = y^* / t^*$ to \eqref{opt:Q1}, which by Lemma \ref{lemma:Q0_eq_Q1} is also optimal for \eqref{opt:Q0}. As noted above, the policy $\pi^*(a | s) = \lambda^*_{sa} / \sum_{a'} \lambda^*_{sa'}$ thus minimizes the OIR over the MDP $(\mc{S}, \mc{A}, p, c)$. This proves Theorem \ref{thm:Q0_eq_Q0_concave}, completing our derivation of the concave transformation of \eqref{opt:Q0}.




\subsection{Proof of Theorem \ref{thm:stationarity_implies_global_optimality_info_ratio}}

% \begin{theorem} \label{thm:stationarity_implies_global_optimality_info_ratio}
%     Let Assumptions \ref{assum:actor_conditions} and \ref{assum:hidden_concavity_info_ratio} hold. Let $\theta^*$ be a stationary point of \eqref{stat_implies_glob:1}, i.e.
%     %
%     \begin{align}
%         \nabla \rho(\theta^*) = 0. \label{eqn:theta_stationary_rho}
%     \end{align}
%     %
%     Then $\theta^*$ is globally optimal for \eqref{stat_implies_glob:1}.
% \end{theorem}
%
%
%
%
%
\begin{proof}

The key idea behind the proof is to show that the stationary point $\theta^*$ corresponds to an optimal solution to the concave program \eqref{opt:Q3} and thus also provides an optimal solution to the quasiconvex OIR minimization problem \eqref{opt:Q0}. To do this we first reinterpret \eqref{stat_implies_glob:1} as a concave program via the perspective transformation considered in \S\ref{sec:concave_program_2}. We then demonstrate that the feasible solution corresponding to $\theta^*$ is a stationary point of this concave program and thus a global optimal solution of the problem. This will imply that $\theta^*$ is optimal for \eqref{stat_implies_glob:1}.
%
The proof builds on that of Thm.~4.2 of \cite{zhang2020variational}, with key modifications to accommodate the fact that the underlying OIR optimization problem is not convex, but \textit{quasiconvex} in the state-action occupancy measure.

We first reformulate \eqref{stat_implies_glob:1} as a maximization problem. Let $q(\theta) = 1 / \rho(\theta) = (\kappa + H(d_{\theta})) / J(\theta)$. Notice that $\widehat{H}(\lambda_{\theta}) = H(d_{\theta})$, where $\widehat{H}(\lambda) = H(d^{\lambda})$ is the entropy of the state occupancy measure $d^{\lambda} \in \mc{D}(\mathcal{S})$ given by $d^{\lambda}_s = \sum_a \lambda_{sa}$. Also recall that $J(\theta) = c^T \lambda_{\theta}$, for some vector $c > 0$ of costs. Together, this means that $q(\theta) = (\kappa + \widehat{H}(\lambda_{\theta})) / J(\lambda_{\theta})$. In what follows we prove that $\theta^*$ is globally optimal for $\max_{\theta \in \Theta} q(\theta)$. By Lemma \ref{lemma:Q0_eq_Q1}, this will imply that $\theta^*$ is globally optimal for $\min_{\theta \in \Theta} \rho(\theta)$. A first important fact to notice is that, since $\rho(\theta)$ is strictly positive on $\Theta$, we know $q(\theta)$ is differentiable in $\theta$ and $\nabla q(\theta) = - \nabla \rho(\theta) / [\rho(\theta)]^2$, for all $\theta \in \Theta$. Since $\nabla \rho(\theta^*) = 0$ by assumption, this means $\nabla q(\theta^*) = 0$, so $\theta^*$ is a stationary point of the optimization problem $\max_{\theta \in \Theta} q(\theta)$.

Keeping this in mind, we now reinterpret the problem $\max_{\theta \in \Theta} q(\theta)$ as a related concave program. For $z \in \mathbb{R}^{|\mc{S}| |\mc{A}| + 1}$, let the vector $y \in \mathbb{R}^{|\mc{S}| |\mc{A}|}$ denote all but the last entry in $z$, and let the scalar $t$ denote the last entry of $z$. We will write $z = (y, t)$ for brevity. Let $\zeta : \mc{D}(\mc{S} \times \mc{A}) \rightarrow \mathbb{R}^{|\mc{S}| |\mc{A}| + 1}$ be the mapping given by $\zeta(\lambda) = (\lambda / J(\lambda), 1 / J(\lambda))$. Consider the optimization problems
%
\begin{maxi}
    {\lambda \in \lambda(\Theta)}{\frac{\kappa + \widehat{H}(\lambda)}{J(\lambda)}}{}{}  \label{stat_implies_glob:2}
\end{maxi}
%
and
%
\begin{maxi}
    {z \in (\zeta \circ \lambda)(\Theta)}{ P_{\kappa, \widehat{H}}(z)}{}{}, \label{stat_implies_glob:3}
\end{maxi}
%
where $P_{\kappa, \widehat{H}} : \mathbb{R}^{|\mc{S}| |\mc{A}| + 1} \rightarrow \mathbb{R}$ denotes the perspective transformation of $\kappa + \widehat{H}(\lambda)$, given by $P_{\kappa + \widehat{H}} (z) = P_{\kappa, \widehat{H}} ((y, t)) = t ( \kappa + \widehat{H}(y / t))$. For notational convenience we henceforth drop the dependency on $\kappa$ and simply write $P_{\widehat{H}}$ and $\widehat{H}$ instead of $P_{\kappa, \widehat{H}}$ and $\kappa + \widehat{H}$. Recall that, since $\widehat{H}$ is concave over the region $\mc{D}(\mc{S} \times \mc{A})$, its perspective transform $P_{\widehat{H}}$ is concave over the region $\zeta(\mc{D}(\mc{S} \times \mc{A}))$. $P_{\widehat{H}}$ is thus concave over the convex, compact region $(\zeta \circ \lambda)(\Theta) \subseteq \zeta(\mc{D}(\mc{S} \times \mc{A}))$.

Our goal is to show that $\theta^*$ corresponds to a stationary point of the concave program \eqref{stat_implies_glob:3}. To see why this suffices, consider the following. Clearly if $\lambda^* = \lambda(\theta^*)$ is globally optimal for \eqref{stat_implies_glob:2}, then $\theta^*$ is globally optimal for \eqref{stat_implies_glob:1}. Notice that the problem \eqref{stat_implies_glob:2} is quasiconcave, as the objective is quasiconcave and the feasible region is convex and compact. Furthermore, since $\widehat{H}$ is concave and $J$ is linear and strictly positive in $\lambda$, the optimization problem \eqref{stat_implies_glob:3} is the concave transformation of problem \eqref{stat_implies_glob:2} by the discussion in \S\ref{sec:concave_program_2}; this means that any optimal solution $z^*$ of \eqref{stat_implies_glob:3} is both globally optimal for \eqref{stat_implies_glob:3} and allows us to recover a solution $\lambda^* = \zeta^{-1}(z^*)$ that is globally optimal for \eqref{stat_implies_glob:2} and thus \eqref{stat_implies_glob:1}. To prove the theorem, it thus suffices to prove that $z^* = (\zeta \circ \lambda)(\theta^*)$ is globally optimal for \eqref{stat_implies_glob:3}.

The remainder of the proof provides the technical details demonstrating that $z^*$ is a stationary point of \eqref{stat_implies_glob:3}. We first show that the conditions of Assumption \ref{assum:hidden_concavity_info_ratio} can be extended to the mapping $\zeta \circ \lambda$, then use these properties to make a series of bounding arguments that ultimately prove the stationarity of $z^*$. In order to complete the first task of extending the conditions of Assumption \ref{assum:hidden_concavity_info_ratio} to $\zeta \circ \lambda$, we need to prove the following:
%
% \indent (i) $\zeta \circ \lambda$ gives a bijection between $\Theta$ and $(\zeta \circ \lambda)(\Theta)$; \\
% %
% \indent (ii) $\zeta \circ \lambda$ has a Lipschitz continuous inverse; and \\
% %
% \indent (iii) the Jacobian $\nabla_{\theta}(\zeta \circ \lambda)(\theta)$ is Lipschitz. \\
%
\begin{enumerate}[(i)]
    \item $\zeta \circ \lambda$ gives a bijection between $\Theta$ and $(\zeta \circ \lambda)(\Theta)$;
    %
    \item $\zeta \circ \lambda$ has a Lipschitz continuous inverse; and
    %
    \item the Jacobian $\nabla_{\theta}(\zeta \circ \lambda)(\theta)$ is Lipschitz.
\end{enumerate}
%
We first prove (i) and (ii). Given Assumption \ref{assum:hidden_concavity_info_ratio}, this boils down to showing that $\zeta(\lambda) = (\lambda / J(\lambda), 1 / J(\lambda))$ gives a bijection between $\lambda(\Theta)$ and $(\zeta \circ \lambda)(\Theta)$ and that $\zeta$ has a Lipschitz continuous inverse. $\zeta$ is a surjection onto $(\zeta \circ \lambda)(\Theta)$ by definition, so we just need to show it is injective. Fix $\lambda \neq \lambda'$. If $J(\lambda) = J(\lambda')$, then $\lambda / J(\lambda) \neq \lambda' / J(\lambda')$, so $\zeta(\lambda) \neq \zeta(\lambda')$. If $J(\lambda) \neq J(\lambda')$, on the other hand, then $1 / J(\lambda) \neq 1 / J(\lambda')$, so again $\zeta(\lambda) \neq \zeta(\lambda')$. Therefore $\zeta$ is injective and thus gives a bijection. The inverse of $\zeta$ is clearly $\zeta^{-1}(z) = \zeta^{-1}((y, t)) = y / t$. Note that $0 < \min_i c_i \leq t \leq \max_i c_i < \infty$, so $\zeta^{-1}$ has continuous, bounded partial derivatives and is thus Lipschitz continuous on $(\zeta \circ \lambda)(\Theta)$. Combined with Assumption \ref{assum:hidden_concavity_info_ratio}, this implies that $\zeta \circ \lambda$ gives a bijection between $\Theta$ and $(\zeta \circ \lambda)(\Theta)$, proving (i). Since the composition of Lipschitz functions is Lipschitz, $k = (\zeta \circ \lambda)^{-1} = \lambda^{-1} \circ \zeta^{-1}$ is Lipschitz continuous, proving (ii).

For (iii), an application of the chain rule gives $\nabla_{\theta}(\zeta \circ \lambda)(\theta) = \left[ \nabla_{\lambda} \zeta( \lambda(\theta) ) \right]^T \nabla_{\theta} \lambda(\theta)$. Clearly $\nabla_{\lambda} \zeta( \lambda )$ is Lipschitz continuous and bounded over the compact set $\Theta$. Since $\lambda(\theta)$ is Lipschitz by the fact that $\nabla_{\theta} \lambda(\theta)$ is (Lipschitz) continuous and bounded over $\Theta$, this implies that $\nabla_{\lambda} \zeta( \lambda(\theta) )$ is Lipschitz and bounded on $\theta \in \Theta$. Furthermore, $\nabla_{\theta} \lambda(\theta)$ is Lipschitz by assumption and bounded over $\Theta$, so all entries in the matrix product $\left[ \nabla_{\lambda} \zeta( \lambda(\theta) ) \right]^T \nabla_{\theta} \lambda(\theta)$ are sums and products of Lipschitz, bounded functions over $\Theta$, implying that $\nabla_{\theta}(\zeta \circ \lambda)(\theta)$ is Lipschitz on $\Theta$, which proves (iii).

We now move on to the bounding arguments that will ultimately prove that $z^*$ is a stationary point of \eqref{stat_implies_glob:3}. First, notice that
%
$$(P_{\widehat{H}} \circ \zeta \circ \lambda)(\theta) = P_{\widehat{H}}(\zeta(\lambda(\theta))) = \frac{\kappa + \widehat{H}(\lambda(\theta))}{J(\lambda(\theta))} = \frac{\kappa + \widehat{H}(\lambda_{\theta})}{J(\lambda_{\theta})} = q(\theta),$$
%
%
so $\nabla_{\theta} (P_{\widehat{H}} \circ \zeta \circ \lambda)(\theta^*) = \nabla_{\theta} \frac{\kappa + \widehat{H}(\lambda_{\theta^*})}{J(\lambda_{\theta^*})} = \nabla q(\theta^*) = 0$. Since $P_{\widehat{H}}$ is concave and locally Lipschitz on $(\zeta \circ \lambda)(\Theta)$, by the chain rule we have
%
$$\nabla_{\theta} (P_{\widehat{H}} \circ \zeta \circ \lambda)(\theta^*) = \left[ \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) \right]^T \nabla_z P_{\widehat{H}}(z^*) = 0,$$
%
where $z^* = (\zeta \circ \lambda)(\theta^*)$.
%
%
This trivially implies that, for all $\theta \in \Theta$,
%
\begin{align} \label{stat_implies_glob:4}
    \langle \nabla_z P_{\widehat{H}}(z^*), \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) (\theta - \theta^*) \rangle = \langle \left[ \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) \right]^T \nabla_z P_{\widehat{H}}(z^*), \theta - \theta^* \rangle = 0.
\end{align}
%
Equation \eqref{stat_implies_glob:4} is important to the bounding arguments presented next.

In the following equations, let $\theta = k(z)$ and $\theta^* = k(z^*)$. Adding and subtracting $\langle \nabla_z P_{\widehat{H}}(z^*), \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) (\theta - \theta^*)$, using equation \eqref{stat_implies_glob:4}, and applying the Cauchy-Schwarz inequality, we get
%
\begin{align}
    \langle \nabla_z P_{\widehat{H}}(z^*), z - z^* \rangle &= \langle \nabla_z P_{\widehat{H}}(z^*), (\zeta \circ \lambda)(\theta) - (\zeta \circ \lambda)(\theta^*) \rangle \\
    %
    &= \langle \nabla_z P_{\widehat{H}}(z^*), \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) (\theta - \theta^*) \rangle \nonumber \\
    %
    & \hspace{5mm} + \langle \nabla_z P_{\widehat{H}}(z^*), (\zeta \circ \lambda)(\theta) - (\zeta \circ \lambda)(\theta^*) - \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) (\theta - \theta^*) \rangle \\
    %
    &= \langle \nabla_z P_{\widehat{H}}(z^*), (\zeta \circ \lambda)(\theta) - (\zeta \circ \lambda)(\theta^*) - \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) (\theta - \theta^*) \rangle \\
    %
    &\leq \norm{\nabla_z P_{\widehat{H}}(z^*)} \norm{(\zeta \circ \lambda)(\theta) - (\zeta \circ \lambda)(\theta^*) - \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) (\theta - \theta^*) }.
\end{align}
%
Since $\nabla_{\theta} (\zeta \circ \lambda)(\theta)$ is Lipschitz, there exists $K_0 > 0$ such that
%
\begin{align*}
    \norm{(\zeta \circ \lambda)(\theta) - (\zeta \circ \lambda)(\theta^*) - \nabla_{\theta} (\zeta \circ \lambda)(\theta^*) (\theta - \theta^*)} \leq \frac{K_0}{2} \norm{\theta - \theta^*}^2.
\end{align*}
%
In addition, $k = (\zeta \circ \lambda)^{-1}$ is Lipschitz, so there exists $K_1 > 0$ such that
%
\begin{align*}
    \norm{\theta - \theta^*}^2 = \norm{k(z) - k(z^*)}^2 \leq K_1^2 \norm{z - z^*}^2.
\end{align*}
%
Combining these inequalities yields that
%
\begin{align}
    \langle \nabla_z P_{\widehat{H}}(z^*), z - z^* \rangle \leq \frac{K_0 K_1^2}{2} \norm{\nabla_z P_{\widehat{H}}(z^*)} \norm{z - z^*}^2, \text{ for all } z \in (\zeta \circ \lambda)(\Theta).
\end{align}
%
Since $(\zeta \circ \lambda)(\Theta)$ is convex, we can replace $z$ above with $(1 - \alpha) z^* + \alpha z$ for any $\alpha \in [0, 1]$, which gives
%
\begin{align*}
    \alpha \langle \nabla_z P_{\widehat{H}}(z^*), z - z^* \rangle \leq \frac{K_0 K_1^2 \alpha^2}{2} \norm{\nabla_z P_{\widehat{H}}(z^*)} \norm{z - z^*}^2, \text{ for all } z \in (\zeta \circ \lambda)(\Theta) \text{ and all } \alpha \in [0, 1].
\end{align*}
%
Dividing both sides by $\alpha$ and taking the limit as $\alpha$ approaches 0 from above, we obtain
%
\begin{align*}
    \langle \nabla_z P_{\widehat{H}}(z^*), z - z^* \rangle \leq 0, \text{ for all } z \in (\zeta \circ \lambda)(\Theta).
\end{align*}
%
Since problem \eqref{stat_implies_glob:3} is concave in $z$, this implies that $z^* = (\zeta \circ \lambda)(\theta^*)$ is a stationary point of that problem. The solution $z^*$ is therefore a global optimal solution to \eqref{stat_implies_glob:3}, which completes the proof.
\end{proof}


\subsection{Proof of Theorem \ref{thm:OIR_convergence_rate}}
% %
% \begin{theorem} \label{thm:OIR_convergence_rate}
%     Let Assumptions % \ref{assum:actor_conditions},
%     \ref{assum:actor_conditions},
%     \ref{assum:hidden_concavity_info_ratio},
%     % \ref{assum:OIR_exact_gradients},
%     and \ref{assum:OIR_lipschitz_jacobian} hold. Let $D_{\zeta} = \max_{z, z' \in (\zeta \circ \lambda)(\Theta)} \norm{z - z'}$ denote the diameter of the convex, compact set $(\zeta \circ \lambda)(\Theta)$. Define $M = \max_{\theta \in \Theta} \rho(\theta)$, $m = \min_{\theta \in \Theta} \rho(\theta)$, $K = \max \{ m^2 L, M^2 m^2 L \}$, and $L_1 = \max \{ L, M^2 L \}$. Then, with $\eta = 1 / K$, we have, for all $t \geq 0$,
%     %
%     \begin{equation} \label{ineq:OIR_prox_bound}
%         \rho(\theta_t) - \rho(\theta^*) \leq \frac{ 4 M^2 L_1 \ell^2 D^2_{\zeta}}{t + 1}.
%     \end{equation}
% \end{theorem}
%
\begin{proof}
The key idea behind the proof is to link the objective function $\rho(\theta)$ that the updates \eqref{eqn:prox_update_rho} are minimizing to the concave structure of the transformed problem \eqref{opt:Q3}. This will allow us to derive the bound \eqref{ineq:OIR_prox_bound} by studying related bounds for the concave objective function of \eqref{opt:Q3}. The proof proceeds as follows: first, we convert the descent scheme \eqref{eqn:prox_update_rho} to an equivalent ascent scheme; next, we link the objective that this ascent scheme is maximizing to the objective function of \eqref{opt:Q3}; third, we derive a sequence capturing the convergence rate of the ascent scheme; finally, we relate this sequence back to \eqref{eqn:prox_update_rho} to obtain \eqref{ineq:OIR_prox_bound}.


In order to more easily make the connection to the concave maximization problem \eqref{opt:Q3}, we first transform \eqref{eqn:prox_update_rho} into an equivalent projected gradient \textit{ascent} scheme. Define $q(\theta) = 1 / \rho(\theta) = (\kappa + H(d_{\theta})) / J(\theta)$, and notice that $\nabla q(\theta) = - \nabla \rho(\theta) / \left[ \rho(\theta) \right]^2$. The projected gradient ascent scheme can then be written
%
%
\begin{align}
    \theta_{t+1} &= \text{Proj}_{\Theta} \left( \theta_t - \eta \nabla \rho(\theta_t) \right) \nonumber \\
    %
    &\labelrel={eqn:prox_transform1} \text{Proj}_{\Theta} \left( \theta_t + \eta \left[ \rho(\theta_t) \right]^2 \nabla q(\theta_t) \right) \nonumber \\
    %
    &\labelrel={eqn:prox_transform2} \argmax_{\theta} \left( q(\theta_t) + \left< \nabla q(\theta_t), \theta - \theta_t \right> - \frac{\left[ \rho(\theta_t) \right]^2}{2 \eta} \norm{\theta - \theta_t}^2 \right). \nonumber \\
    %
    &\labelrel={eqn:prox_transform3} \argmax_{\theta} \left( q(\theta_t) + \left< \nabla q(\theta_t), \theta - \theta_t \right> - \frac{1}{2 \eta_t} \norm{\theta - \theta_t}^2 \right), \label{eqn:OIR_prox_ascent}
\end{align}
%
where \eqref{eqn:prox_transform1} follows by noticing that $\nabla \rho(\theta) = - [\rho(\theta)]^2 \nabla q(\theta)$ and making the appropriate substitution, \eqref{eqn:prox_transform2} holds by definition of the $\text{Proj}$ operator, and \eqref{eqn:prox_transform3} results from defining $\eta_t = \eta [\rho(\theta_t)]^2 = [\rho(\theta_t)]^2 / K_0$.

In order to analyze the updates \eqref{eqn:OIR_prox_ascent} and eventually tie the analysis back to \eqref{eqn:prox_update_rho}, we next identify a family $\{ K_c \ | \ c \in [m, M] \}$ of Lipschitz constants of the gradient $\nabla q(\theta)$. By Assumption \ref{assum:OIR_lipschitz_jacobian}, $\nabla q(\theta)$ is Lipschitz and $\norm{ \nabla q(\theta) - \nabla q(\theta')} \leq L_0 \norm{\theta - \theta'}$, for all $\theta, \theta' \in \Theta$, where $L_0 = m^2 L$. Let $K = \max \{ L_0, M^2 L_0 \} = \max \{ m^2 L, M^2 m^2 L \}$. Then, for all scalars $c \in [m , M]$, $\nabla q(\theta)$ satisfies $\norm{ \nabla q(\theta) - \nabla q(\theta')} \leq K_c \norm{\theta - \theta'},$ where $K_c = K / c^2$ is the desired Lipschitz constant. These will be critical in the analysis to follow.

We now link the updates \eqref{eqn:OIR_prox_ascent} and objective function $q(\theta)$ to \eqref{opt:Q3}, then study a related sequence to capture the convergence rate of \eqref{eqn:OIR_prox_ascent}.
%
The overall goal is to study the sequence $\alpha_t = \left[ q(\theta^*) - q(\theta_t) \right] / 2 K_m \ell^2 D^2_{\zeta}$, for $t \geq 0$, ultimately using properties of the sequence to show that $q(\theta^*) - q(\theta_t) \leq 4 K_m \ell^2 D^2_{\zeta} / (1 + t)$, for all $t \geq 0$. We will then use this inequality to obtain the desired bound \eqref{ineq:OIR_prox_bound}.
%
The remainder of the proof proceeds along lines similar to that of Thm.~4.4 in \cite{zhang2020variational}, but with modifications to accommodate the use of the perspective transform, the variable transformation $\zeta$, and the non-constant stepsizes $\eta_t = \eta [ \rho(\theta_t)]^2$.
%

Before proceeding, we make some necessary definitions. Define $\widehat{H}(\lambda) = H(d^{\lambda})$, where $H(d^{\lambda})$ is the entropy of the state occupancy measure $d^{\lambda}(s) = \sum_a \lambda(s, a)$ corresponding to the state-action occupancy measure $\lambda \in \mc{D}(\mc{S} \times \mc{A})$. For a given $\kappa \geq 0$, let $P_{\kappa, \widehat{H}} : \mathbb{R}^{|\mc{S}| |\mc{A}| + 1} \rightarrow \mathbb{R}$ denote the perspective transformation of $\kappa + \widehat{H}(\lambda)$, given by $P_{\kappa + \widehat{H}} (z) = P_{\kappa, \widehat{H}} ((y, t)) = t ( \kappa + \widehat{H}(y / t))$. For notational convenience we henceforth drop the dependency on $\kappa$ and simply write $P_{\widehat{H}}$.

Our next step is to make use of the concave structure of $P_{\widehat{H}}$, $\zeta \circ \lambda$, and the associated problem \eqref{opt:Q3} to derive properties that will aid our analysis of $\{ \alpha_t \}_{t \in \mathbb{N}}$. We will first spend some time deriving several useful inequalities regarding $P_{\widehat{H}}$ and $\zeta \circ \lambda$ before returning to our analysis of $\{ \alpha_t \}_{t \in \mathbb{N}}$. Notice that $q(\theta) = (\kappa + \widehat{H}(\lambda_{\theta})) / J(\lambda_{\theta}) = P_{\widehat{H}}(\zeta(\lambda_{\theta})) = P_{\widehat{H}}((\zeta \circ \lambda)(\theta))$, for all $\theta \in \Theta$. This means that we can rewrite $\alpha_t$ as
%
\begin{equation} \label{eqn:alpha_redef}
    \alpha_t = \left[ P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) \right] / 2 K_m \ell^2 D^2_{\zeta}.
\end{equation}
%
Recall that $P_{\widehat{H}}$ is concave over the region $\zeta(\mc{D}(\mc{S} \times \mc{A}))$, since $\widehat{H}$ is concave over the region $\mc{D}(\mc{S} \times \mc{A})$ and the perspective transform preserves concavity. $P_{\widehat{H}}$ is thus concave over the convex, compact region $(\zeta \circ \lambda)(\Theta) \subseteq \zeta(\mc{D}(\mc{S} \times \mc{A}))$.
%
Furthermore, since $P_{\widehat{H}}((\zeta \circ \lambda)(\theta)) = q(\theta)$, we have $\nabla P_{\widehat{H}}((\zeta \circ \lambda)(\theta)) = \nabla q(\theta)$, so $\nabla P_{\widehat{H}}((\zeta \circ \lambda)(\theta))$ is $K_c$-Lipschitz, for any $K_c = K / c^2, c \in [m, M]$. This implies (see Lem.~1.2.3 in \cite{nesterov2003introductory}), for any $c \in [m, M]$, that
%
\begin{equation*}
    \Big\rvert P_{\widehat{H}} ((\zeta \circ \lambda)(\theta)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) - \left< \nabla P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)), \theta - \theta_t \right> \Big\rvert \leq \frac{K_c}{2} \norm{\theta - \theta_t}^2,
\end{equation*}
%
whence, for any $\theta \in \Theta$,
%
\begin{align}
    P_{\widehat{H}} ((\zeta \circ \lambda)(\theta)) &\geq P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_t)) + \left< \nabla P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_t)), \theta - \theta_t \right> - \frac{K_c}{2} \norm{\theta - \theta_t}^2 \nonumber \\
    %
    &\geq P_{\widehat{H}} ((\zeta \circ \lambda)(\theta)) - K_c \norm{\theta - \theta_t}^2. \label{ineq:conv1_0} 
\end{align}
%
In light of these inequalities, and using the fact that $\eta_t = [\rho(\theta_t)]^2 / K = 1 / K_{\rho(\theta_t)}$ by setting $c = \rho(\theta_t)$ in the definition of $K_c$, we have
%
\begin{align}
    P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_{t+1})) &\geq P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_t)) + \left< \nabla P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_t)), \theta_{t+1} - \theta_t \right> - \frac{K_{\rho(\theta_t)}}{2} \norm{\theta_{t+1} - \theta_t}^2 \nonumber \\
    %
    &\labelrel={eqn:conv1_1} \max_{\theta \in \Theta} \left( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_t)) + \left< \nabla P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_t)), \theta - \theta_t \right> - \frac{K_{\rho(\theta_t)}}{2} \norm{\theta - \theta_t}^2 \right) \nonumber \\
    %
    &\labelrel\geq{ineq:conv1_2} \max_{\theta \in \Theta} \left( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta)) - K_{\rho(\theta_t)} \norm{\theta - \theta_t}^2 \right) \nonumber \\
    %
    &\labelrel\geq{ineq:conv1_3} \max_{\theta \in \Theta} \left( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta)) - K_m \norm{\theta - \theta_t}^2 \right) \nonumber \\
    %
    &\labelrel\geq{ineq:conv1_4} \max_{\alpha \in [0, 1]} \{ P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_{\alpha})) - K_m \norm{\theta_{\alpha} - \theta_t}^2 \ \big\rvert \ \theta_{\alpha} = k \big( \alpha (\zeta \circ \lambda)(\theta^*) + (1 - \alpha) (\zeta \circ \lambda)(\theta_t) \big) \}, \label{ineq:OIR_prox_conv_rate1}
\end{align}
%
where \eqref{eqn:conv1_1} follows from the optimality of the update \eqref{eqn:OIR_prox_ascent}, \eqref{ineq:conv1_2} holds by \eqref{ineq:conv1_0}, \eqref{ineq:conv1_3} follows from the fact that $K_{\rho(\theta_t)} \leq K_m$, the \eqref{ineq:conv1_4} follows by the convexity of $(\zeta \circ \lambda)(\Theta)$. Now notice that
%
\begin{align}
    P_{\widehat{H}}((\zeta \circ \lambda)(\theta_{\alpha})) &= P_{\widehat{H}} \Big( (\zeta \circ \lambda) \big( k(\alpha (\zeta \circ \lambda)(\theta^*) + (1 - \alpha) (\zeta \circ \lambda)(\theta_t)) \big) \Big) \nonumber \\
    %
    &= P_{\widehat{H}}( \alpha (\zeta \circ \lambda)(\theta^*) + (1 - \alpha) (\zeta \circ \lambda)(\theta_t)) \nonumber \\
    %
    &\geq \alpha P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) + (1 - \alpha) P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)), \label{ineq:OIR_prox_conv_rate1_2}
\end{align}
%
where the first equality holds by the definition of $\theta_{\alpha}$ given in \eqref{ineq:OIR_prox_conv_rate1}, the second follows from the fact that $k((\zeta \circ \lambda)(\theta)) = \theta$, for any $\theta \in \Theta$, and the final inequality is yielded by the concavity of $P_{\widehat{H}}$ over $(\zeta \circ \lambda)(\Theta)$.
%
Furthermore,
%
\begin{align}
    \norm{ \theta_{\alpha} - \theta_t }^2 &\labelrel={eqn:conv1_5} \norm{ k(\alpha (\zeta \circ \lambda)(\theta^*) + (1 - \alpha)(\zeta \circ \lambda)(\theta_t)) - k((\zeta \circ \lambda)(\theta_t)) }^2 \nonumber \\
    %
    &\labelrel\leq{ineq:conv1_6} \ell^2 \norm{ \alpha (\zeta \circ \lambda)(\theta^*) + (1 - \alpha)(\zeta \circ \lambda)(\theta_t) - (\zeta \circ \lambda)(\theta_t) }^2 \nonumber \\
    %
    &\leq \alpha^2 \ell^2 \norm{(\zeta \circ \lambda)(\theta^*) - (\zeta \circ \lambda)(\theta_t)}^2 \nonumber \\
    %
    &\labelrel\leq{ineq:conv1_7} \alpha^2 \ell^2 D^2_{\zeta}, \label{ineq:OIR_prox_conv_rate1_3}
\end{align}
%
where \eqref{eqn:conv1_5} holds by the definition of $\theta_{\alpha}$ and the fact that $k((\zeta \circ \lambda)(\theta)) = \theta$, \eqref{ineq:conv1_6} follows since $k$ is $\ell$-Lipschitz, and \eqref{ineq:conv1_7} results from the definition of $D_{\zeta}$ given in the statement of the theorem. Now, the inequalities \eqref{ineq:OIR_prox_conv_rate1}, \eqref{ineq:OIR_prox_conv_rate1_2}, and \eqref{ineq:OIR_prox_conv_rate1_3} combine to yield
%
\begin{align}
    P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) &- P_{\widehat{H}} ( (\zeta \circ \lambda)(\theta_{t+1})) \nonumber \\
    %
    &\labelrel\leq{ineq:conv1_8} \min_{\alpha \in [0, 1]} \{ P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_{\alpha})) + K_m \norm{ \theta_{\alpha} - \theta_t }^2 \nonumber \\ 
    %
    & \hspace{2cm} \big\rvert \ \theta_{\alpha} = k \big( \alpha (\zeta \circ \lambda)(\theta^*) + (1 - \alpha) (\zeta \circ \lambda)(\theta_t) \big) \} \nonumber \\
    %
    &\labelrel\leq{ineq:conv1_9} \min_{\alpha \in [0, 1]} \Big( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) - \alpha P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - (1 - \alpha) P_{\widehat{H}} ((\zeta \circ \lambda)(\theta_t)) + K_m \alpha^2 \ell^2 D^2_{\zeta} \Big) \nonumber \\
    %
    &= \min_{\alpha \in [0, 1]} \Big( (1 - \alpha) \big( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}( (\zeta \circ \lambda)(\theta_t)) \big) + K_m \alpha^2 \ell^2 D^2_{\zeta} \Big), \label{ineq:OIR_prox_conv_rate2}
\end{align}
%
where inequality \eqref{ineq:conv1_8} results from multiplying both sides of \eqref{ineq:OIR_prox_conv_rate1} by $-1$ and adding $P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)$, and \eqref{ineq:OIR_prox_conv_rate1_2} and \eqref{ineq:OIR_prox_conv_rate1_3} together yield \eqref{ineq:conv1_9}.

Now that we have the important inequalities \eqref{ineq:OIR_prox_conv_rate1}, \eqref{ineq:OIR_prox_conv_rate1_2}, \eqref{ineq:OIR_prox_conv_rate1_3}, and \eqref{ineq:OIR_prox_conv_rate2} in hand, we return to our analysis of the sequence $\{ \alpha_t \}_{t \in \mathbb{N}}$ defined in \eqref{eqn:alpha_redef}. Our goal is to derive a useful upper bound for the sequence, then use this bound to prove that, when the iterates $\{ \theta_t \}$ are generated by \eqref{eqn:OIR_prox_ascent}, $q(\theta_t)$ converges to $q(\theta^*)$ at the certain rate. We will then use these results to prove \eqref{ineq:OIR_prox_bound}.

To begin our analysis of the sequence, we use \eqref{ineq:OIR_prox_conv_rate2} to derive a useful recursive inequality for $\{ \alpha_t \}_{t \in \mathbb{N}}$. Notice that $\alpha_t \geq 0$, for all $t \geq 0$. Now, assume that $\alpha_0 \geq 1$. This implies that $P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_0)) \geq 2 K_m \ell^2 D^2_{\zeta}$, so the minimum in \eqref{ineq:OIR_prox_conv_rate2} is attained when $\alpha = 1$. But then $\alpha_1 \leq 1 / 2$. Since this argument is independent of the choice of $t$, we can assume without loss of generality that $\alpha_t \leq 1$, for all $t \geq 0$, by simply discarding $\alpha_0$ if it is greater than 1.

We next show that $\alpha_{t+1} \leq \alpha_t$, for all $t \geq 0$. Since $\alpha_t \leq 1$, $\alpha_t$ is always the minimizer of the right-hand side of \eqref{ineq:OIR_prox_conv_rate2}, which can be seen by setting the derivative with respect to $\alpha$ equal to 0 and solving for $\alpha$. Substituting $\alpha_t$ into \eqref{ineq:OIR_prox_conv_rate2}, we see that
%
\begin{align}
    P_{\widehat{H}}((\zeta &\circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_{t+1})) \nonumber \\
    %
    &\leq \Big( 1 - \frac{ P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) }{2 K_m \ell^2 D^2_{\zeta}} \Big) \big( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}( (\zeta \circ \lambda)(\theta_t)) \big) \nonumber \\
    %
    & \hspace{1cm} + \Big( \frac{ P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) }{2 K_m \ell^2 D^2_{\zeta}} \Big)^2 K_m \ell^2 D^2_{\zeta} \nonumber \\
    %
    &\labelrel={eqn:conv1_10} \Big( 1 - \frac{ P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) }{2 K_m \ell^2 D^2_{\zeta}} \Big) \big( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}( (\zeta \circ \lambda)(\theta_t)) \big) \nonumber \\
    %
    & \hspace{1cm} + \frac{ P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) }{4 K_m \ell^2 D^2_{\zeta}} \big( P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) \big) \nonumber \\
    %
    &\labelrel={eqn:conv1_11} \Big( 1 - \frac{ P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) }{4 K_m \ell^2 D^2_{\zeta}} \Big) \big( P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}( (\zeta \circ \lambda)(\theta_t)) \big), \label{ineq:OIR_prox_conv_rate3}
\end{align}
%
where \eqref{eqn:conv1_10} results by noticing that one of the $K_m \ell^2 D_{\zeta}^2$ terms cancels and \eqref{eqn:conv1_11} can be obtained by factoring out the $P_{\widehat{H}} ((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}( (\zeta \circ \lambda)(\theta_t))$ term and simplifying. Dividing both sides of \eqref{ineq:OIR_prox_conv_rate3} by $2 K_m \ell^2 D_{\zeta}^2$ shows that $\alpha_{t+1} \leq \alpha_t$.

Now, dividing both sides of \eqref{ineq:OIR_prox_conv_rate3} by $4 K_m \ell^2 D^2_{\zeta}$ yields the recursive inequality
%
\begin{align*}
    \frac{\alpha_{t+1}}{2} \leq \Big( 1 - \frac{\alpha_t}{2} \Big) \frac{\alpha_t}{2},
\end{align*}
%
which implies
%
\begin{align*}
    \frac{2}{\alpha_{t+1}} \geq \frac{1}{\big( 1 - \frac{\alpha_t}{2} \big) \frac{\alpha_t}{2}} = \frac{2 \big( 1 - \frac{\alpha_t}{2} \big) + \alpha_t }{\big( 1 - \frac{\alpha_t}{2} \big) \alpha_t} = \frac{2}{\alpha_t} + \frac{1}{1 - \frac{\alpha_t}{2}} \geq \frac{2}{\alpha_t} + 1 \geq \frac{2}{\alpha_0} + t.
\end{align*}
%
Since $\alpha_0 \leq 1$, this gives us that
%
\begin{align}
    \frac{\alpha_{t+1}}{2} \leq \frac{1}{t + \frac{2}{\alpha_0}} \leq \frac{1}{t + 2}. \label{ineq:conv1_12}
\end{align}
%
Multiplying both sides of \eqref{ineq:conv1_12} by $4 K_m \ell^2 D^2_{\zeta}$ finally yields, for all $t \geq 0$,
%
\begin{align}
    q(\theta^*) - q(\theta_t) = P_{\widehat{H}}((\zeta \circ \lambda)(\theta^*)) - P_{\widehat{H}}((\zeta \circ \lambda)(\theta_t)) \leq \frac{4 K_m \ell^2 D^2_{\zeta}}{t + 1}. \label{ineq:conv1_13}
\end{align}
%
We have thus finally obtained our convergence rate result for the projected gradient ascent scheme \eqref{eqn:OIR_prox_ascent}. We now finish the proof by using this result to derive the corresponding rate for the OIR projected gradient descent scheme \eqref{eqn:prox_update_rho}. Since $q(\theta) = 1 / \rho(\theta)$ and $K_m = K / m^2$, \eqref{ineq:conv1_13} implies that
%
\begin{align*}
    \frac{\rho(\theta_t) - \rho(\theta^*)}{M^2} &\leq  \frac{\rho(\theta_t) - \rho(\theta^*)}{\rho(\theta^*) \rho(\theta_t)} = \frac{1}{\rho(\theta^*)} - \frac{1}{\rho(\theta_t)}
    %
    = q(\theta^*) - q(\theta_t) \leq \frac{4 K_m \ell^2 D^2_{\zeta}}{t + 1} = \frac{4 K \ell^2 D^2_{\zeta}}{m^2 (t + 1)}.
\end{align*}
%
Remembering that $K = \max \{ m^2 L, M^2 m^2 L \}$ and letting $L_1 = \max \{ L, M^2 L \}$, we have
%
\begin{equation*}
    \rho(\theta_t) - \rho(\theta^*) \leq \frac{M^2}{m^2} \frac{4 K \ell^2 D^2_{\zeta}}{t + 1} = \frac{4 M^2 L_1 \ell^2 D^2_{\zeta} }{ t + 1 },
\end{equation*}
which completes the proof.
\end{proof}


\subsection{Proof of Theorem \ref{thm:actor_conv}} \label{sec:actor_conv_appendix}


For clarity, we first provide a detailed description of the one-step, iterative version of IDAC analyzed in Theorem \ref{thm:actor_conv}. As mentioned in \S\ref{sec:as_conv}, this version of IDAC results from taking $K = 1$ in Algorithm \ref{alg:irac}, setting $\tau_t = \alpha_t$, for all $t \geq 0$, and including the policy projection \eqref{eqn:irac_projected_policy_update}. Let a parameterized policy class $\{ \pi_{\theta} \}_{\theta \in \Theta}$ and a class $\{ v_{\omega} \}_{\omega \in \Omega}$ of state value function approximators be given. We assume for ease of exposition that the same class $\{ v_{\omega} \}_{\omega \in \Omega}$ of function approximators is used for both the cost and entropy critics, but this assumption can be removed both in practice and in the convergence analysis provided in the subsequent section. Initialize step-size sequences $\{ \alpha_t \}, \{ \beta_t \},$ and policy parameter $\theta_0$ as above. Initialize the cost and entropy critic parameters $\omega^J_0$ and $\omega^H_0$, respectively, as well as constants $\mu^J_{-1}, \mu^H_{-1} > 0$. At timestep $t$, call $d_{\theta_t} = \textsc{DensityEstimator}(\theta_t)$, then update the moving averages corresponding to the cost and entropy estimates via
%
\begin{equation} \label{eqn:irac_mu_j_update}
    \mu^J_t = (1 - \tau_t) \mu^J_{t-1} + \tau_t c(s_t, a_t),
\end{equation}
%
\begin{equation} \label{eqn:irac_mu_h_update}
\mu^H_t = (1 - \tau_t) \mu^H_{t-1} - \tau_t \log d_{\theta_t}(s_t).
\end{equation}
%
Next, update the cost and entropy TD errors
%
%
\begin{equation} \label{eqn:irac_delta_j_update}
\delta^J_t = c(s_t, a_t) - \mu^J_t + v_{\omega^J_t}(s_{t+1}) - v_{\omega^J_t}(s_t),
\end{equation}
%
\begin{equation} \label{eqn:irac_delta_h_update}
\delta^H_t = - \log d_{\theta_t}(s_t) - \mu^H_t + v_{\omega^H_t}(s_{t+1}) - v_{\omega^H_t}(s_t),
\end{equation}
%
and perform the corresponding critic updates
%
\begin{equation} \label{eqn:irac_j_critic_update}
\omega^J_{t+1} = \omega^J_t + \alpha_t \delta^J_t \nabla v_{\omega^J_t}(s_t),
\end{equation}
%
\begin{equation} \label{eqn:irac_h_critic_update}
\omega^H_{t+1} = \omega^H_t + \alpha_t \delta^H_t \nabla v_{\omega^H_t}(s_t).
\end{equation}
%
Finally, carry out the projected actor update \eqref{eqn:irac_projected_policy_update}, restated here for convenience:
%
\begin{equation*} % \label{eqn:irac_policy_update}
% \theta_{t+1} = \theta_t - \beta_t \frac{ \delta^J_t (\kappa + \mu^H_t) - \mu^J_t \delta^H_t }{ \left( \kappa + \mu^H_t \right)^2 } \nabla \log \pi_{\theta_t}(a_t | s_t).
\theta_{t+1} = \Gamma \left( \theta_t - \beta_t \frac{ \delta^J_t (\kappa + \mu^H_t) - \mu^J_t \delta^H_t }{ \left( \kappa + \mu^H_t \right)^2 } \nabla \log \pi_{\theta_t}(a_t | s_t) \right).
\end{equation*}

The iterative algorithm just given is what we study in the following convergence analysis. Our analysis leverages the average-reward actor-critic results in \cite{bhatnagar2009natural} as well as the results for ratio optimization actor-critic in \cite{suttle2021reinforcement}. For a given policy parameter $\theta$, let 
$D_\theta = \text{diag} ( d_{\theta} ) \in \mathbb{R}^{| \mathcal{S} | \times | \mathcal{S} |}$ denote the matrix with the elements of $d_{\theta}$ along the diagonal and zeros everywhere else. Define the state cost vector for the average-cost MDP $(\mathcal{S}, \mathcal{A}, p, c)$ to be $c_\theta = [c_{\theta}(s)]_{ s \in \mathcal{S} }^\top \in \mathbb{R}^{| \mathcal{S} |}$, where $c_\theta(s) = \sum_{a \in \mathcal{A}}\pi_\theta(a | s) c(s, a)$. Similarly, let $r_\theta = [- \log d_{\theta}(s)]_{ s \in \mathcal{S} }^\top \in \mathbb{R}^{| \mathcal{S} |}$ denote the state reward vector for the shadow MDP $(\mathcal{S}, \mathcal{A}, p, r)$, where $r(s, a) = - \log d_{\theta}(s)$. Note that the ergodicity condition of Assumption \ref{assum:actor_conditions} implies that $d_{\theta}(s) > 0$, for all $s \in \mathcal{S}, \theta \in \Theta$, so $r(s, a)$ is always defined and finite. Finally, let $P_\theta \in \mathbb{R}^{| \mathcal{S} | \times | \mathcal{S} |}$  denote the state transition probability matrix under policy $\pi_\theta$, i.e., $P_{\theta} ( s' |  s) = \sum_{a \in \mathcal{A} } \pi_{\theta} ( a | s) p(s' | s, a)$, for any $s, s' \in \mathcal{S}$.  
We first show convergence of the critics.

% To ease the burden on the reader, we provide restatements of Lemma \ref{lemma:critics} and Theorem \ref{thm:actor_conv} in terms of equations \eqref{eqn:irac_mu_j_update}-\eqref{eqn:irac_h_critic_update}, \eqref{eqn:irac_projected_policy_update} at the beginning of their respective sections.

% \subsubsection{Proof of Lemma \ref{lemma:critics}}

% \begin{customlemma}{\ref{lemma:critics}}
% Under Assumption \ref{assum:critic_conditions}, given a fixed policy parameter $\theta \in \Theta$, the recursive updates \eqref{eqn:irac_mu_j_update}-\eqref{eqn:irac_h_critic_update} converge as follows: $\lim_{t \rightarrow \infty} \mu^J_t = J(\theta)$ a.s., $\lim_{t \rightarrow \infty} \mu^H_t = H(d_{\theta})$ a.s., $\lim_{t \rightarrow \infty} \omega^J_t = \omega^J_{\theta}$ a.s., and $\lim_{t \rightarrow \infty} \omega^H_t = \omega^H_{\theta}$ a.s., where $\omega^J_{\theta}$ and $\omega^H_{\theta}$ are, respectively, the unique solutions to
% \small
% \begin{align}
% \Phi^{ \top } D_{\theta} \big[ c_{\theta} - J(\theta) \cdot \bm{1} + P_\theta( \Phi \omega^J ) - \Phi \omega^J \big] & = \bm{0}, \label{eqn:td_cost_fixed_point} \\
% %
% \Phi^{ \top } D_{\theta} \big[ r_{\theta} - H(d_{\theta}) \cdot \bm{1} + P_\theta( \Phi \omega^H ) - \Phi \omega^H \big] & = \bm{0}. \label{eqn:td_entropy_fixed_point}
% \end{align}
% \normalsize
% \end{customlemma}

\begin{lemma} \label{lemma:critics}
    Under Assumption \ref{assum:critic_conditions}, given a fixed policy parameter $\theta \in \Theta$, the recursive updates \eqref{eqn:irac_mu_j_update}-\eqref{eqn:irac_h_critic_update} converge as follows: $\lim_{t \rightarrow \infty} \mu^J_t = J(\theta)$ a.s., $\lim_{t \rightarrow \infty} \mu^H_t = H(d_{\theta})$ a.s., $\lim_{t \rightarrow \infty} \omega^J_t = \omega^J_{\theta}$ a.s., and $\lim_{t \rightarrow \infty} \omega^H_t = \omega^H_{\theta}$ a.s., where $\omega^J_{\theta}$ and $\omega^H_{\theta}$ are, respectively, the unique solutions to
    \small
    \begin{align}
    \Phi^{ \top } D_{\theta} \big[ c_{\theta} - J(\theta) \cdot \bm{1} + P_\theta( \Phi \omega^J ) - \Phi \omega^J \big] & = \bm{0}, \label{eqn:td_cost_fixed_point} \\
    %
    \Phi^{ \top } D_{\theta} \big[ r_{\theta} - H(d_{\theta}) \cdot \bm{1} + P_\theta( \Phi \omega^H ) - \Phi \omega^H \big] & = \bm{0}. \label{eqn:td_entropy_fixed_point}
    \end{align}
    \normalsize
\end{lemma}

% \begin{lemma}\label{lemma:critics}
% Under Assumption \ref{assum:critic_conditions}, given a fixed policy parameter $\theta \in \Theta$, the recursive updates \eqref{eqn:irac_mu_j_update}-\eqref{eqn:irac_h_critic_update} converge as follows: $\lim_{t \rightarrow \infty} \mu^J_t = J(\theta)$ a.s., $\lim_{t \rightarrow \infty} \mu^H_t = H(d_{\theta})$ a.s., $\lim_{t \rightarrow \infty} \omega^J_t = \omega^J_{\theta}$ a.s., and $\lim_{t \rightarrow \infty} \omega^H_t = \omega^H_{\theta}$ a.s., where $\omega^J_{\theta}$ and $\omega^H_{\theta}$ are, respectively, the unique solutions to
% \small
% \begin{align}
% \Phi^{ \top } D_{\theta} \big[ c_{\theta} - J(\theta) \cdot \bm{1} + P_\theta( \Phi \omega^J ) - \Phi \omega^J \big] & = \bm{0}, \label{eqn:td_cost_fixed_point} \\
% %
% \Phi^{ \top } D_{\theta} \big[ r_{\theta} - H(d_{\theta}) \cdot \bm{1} + P_\theta( \Phi \omega^H ) - \Phi \omega^H \big] & = \bm{0}. \label{eqn:td_entropy_fixed_point}
% \end{align}
% \normalsize
% \end{lemma}

\begin{proof}
Since the policy $\pi_{\theta}$ is held fixed and the shadow MDP reward $- \log d_{\theta}(s)$ can be exactly evaluated, for any $s \in \mathcal{S}$, the proof of Lem.~4 in \cite{bhatnagar2009natural} can be applied separately to the average-cost recursions \eqref{eqn:irac_mu_j_update}, \eqref{eqn:irac_delta_j_update}, \eqref{eqn:irac_j_critic_update} and the shadow MDP recursions \eqref{eqn:irac_mu_h_update}, \eqref{eqn:irac_delta_h_update}, \eqref{eqn:irac_h_critic_update} to obtain the result.
\end{proof}

As in Lem.~5 of \cite{bhatnagar2009natural}, this result shows that the sequences $\{ \omega^J_t \}$ and $\{ \omega^H_t \}$ converge a.s. to the limit points $\omega^J_{\theta}$ and $\omega^H_{\theta}$ of the TD(0) algorithm with linear function approximation for their respective MDPs.
%
%
Due to the use of linear function approximation, when used in the policy update step the value function estimates $v^J_{\theta} = \Phi \omega^J_{\theta}$ and $v^H_{\theta} = \Phi \omega^H_{\theta}$ may result in biased gradient estimates. Similar to the bias characterization given in Lem.~4 in \cite{bhatnagar2009natural}, this bias can be characterized as follows.

% \subsubsection{Proof of Lemma \ref{lemma:bias_pg}}

\begin{lemma}\label{lemma:bias_pg}
	Fix $\theta\in\Theta$. Let
	\small
	\begin{align*}
	%
	\delta^{\theta, J}_t &= c(s_t, a_t) - J(\theta) + \phi(s_{t+1})^\top \omega^J_{\theta} - \phi(s_t)^\top \omega^J_{\theta}, \\
	%
	\delta^{\theta, H}_t &= - \log d_{\theta}(s_t) - H(d_{\theta}) + \phi(s_{t+1})^\top \omega^H_{\theta} - \phi(s_t)^\top \omega^H_{\theta},
	%
	\end{align*}
	\normalsize
	denote the stationary estimates of the TD-errors at time $t$. Let
	\small
	\begin{align*}
	\overline{v}^J_{\theta} &= \mathbb{E}_{\pi_{\theta}} \Big[ c(s,a) - J(\theta) + \phi(s')^\top \omega^J_{\theta} \Big], \\
	%
	\overline{v}^H_{\theta} &= \mathbb{E}_{\pi_{\theta}} \Big[ - \log d_{\theta}(s) - H(d_{\theta}) + \phi(s')^\top \omega^H_{\theta} \Big],
	\end{align*}
	\normalsize
	%
	and let
	\begin{align*}
	    \epsilon^J_{\theta} &= \sum_{s \in \mathcal{S}} d_{\theta}(s) \left[ \nabla_{\theta} \overline{v}^J_{\theta}(s) - \nabla_{\theta} \phi(s)^{\top} \omega^J_{\theta} \right] \\
	    %
	    \epsilon^H_{\theta} &= \sum_{s \in \mathcal{S}} d_{\theta}(s) \left[ \nabla_{\theta} \overline{v}^H_{\theta}(s) - \nabla_{\theta} \phi(s)^{\top} \omega^H_{\theta} \right].
	\end{align*}
	%
	We then have that
	\small
	\begin{align*}
	\mathbb{E}_{\pi_{\theta}} \left[ \frac{ \delta^{\theta, J}_t \left[ \kappa + H(d_{\theta}) \right] - J(\theta) \delta^{\theta, H}_t}{ \left[ \kappa + H(d_{\theta}) \right]^2} \nabla \log \pi_{\theta}(a_t | s_t) \right] = \nabla \rho(\theta) + \frac{ \epsilon^J_{\theta} \left[ \kappa + H(d_{\theta}) \right] - J(\theta) \epsilon^H_{\theta}}{ \left[ \kappa + H(d_{\theta}) \right]^2}.
	\end{align*}
	\normalsize
\end{lemma}
%
\begin{proof}
By Lem.~4 of \cite{bhatnagar2009natural} and Theorem \ref{thm:entropy_gradient},
%
\begin{align*}
    \mathbb{E}_{\pi_{\theta}} \left[ \delta^{\theta, J}_t \nabla \log \pi_{\theta}(a_t | s_t) \right] &= \nabla J(\theta) + \epsilon^J_{\theta}, \\
    %
    \mathbb{E}_{\pi_{\theta}} \left[ \delta^{\theta, H}_t \nabla \log \pi_{\theta}(a_t | s_t) \right] &= \nabla H(d_{\theta}) + \epsilon^H_{\theta}.
\end{align*}
%
This implies that
%
\begin{align*}
    \mathbb{E}_{\pi_{\theta}} & \left[ \frac{ \delta^{\theta, J}_t \left[ \kappa + H(d_{\theta}) \right] - J(\theta) \delta^{\theta, H}_t}{ \left[ \kappa + H(d_{\theta}) \right]^2} \nabla \log \pi_{\theta}(a_t | s_t) \right] \\
    %
    &= \frac{ \left[ \kappa + H(d_{\theta}) \right] \mathbb{E}_{\pi_{\theta}} \left[ \delta^{\theta, J}_t \nabla \log \pi_{\theta}(a_t | s_t) \right] - J(\theta) \mathbb{E}_{\pi_{\theta}} \left[ \delta^{\theta, H}_t \nabla \log \pi_{\theta}(a_t | s_t) \right]}{ \left[ \kappa + H(d_{\theta}) \right]^2 } \\
    %
    &= \frac{ \left[ \kappa + H(d_{\theta}) \right] \left( \nabla J(\theta) + \epsilon^J_{\theta} \right) - J(\theta) \left( \nabla H(d_{\theta}) + \epsilon^H_{\theta} \right) }{ \left[ \kappa + H(d_{\theta}) \right]^2 } \\
    %
    &= \nabla \rho(\theta) + \frac{ \epsilon^J_{\theta} \left[ \kappa + H(d_{\theta}) \right] - J(\theta) \epsilon^H_{\theta}}{ \left[ \kappa + H(d_{\theta}) \right]^2},
\end{align*}
which completes the proof.
\end{proof}

Now we are ready to establish the convergence of the actor step, and thus the actor-critic algorithm. Given any continuous function $f : \Theta \to \mathbb{R}^d$, define the function $\hat{\Gamma}(\cdot)$ using the projection operator $\Gamma$ to be
%
\begin{equation} \label{eqn:gamma_projection_def}
    \hat{\Gamma}(f(\theta))=\lim_{\eta \rightarrow 0^+} \left [ \Gamma(\theta+\eta \cdot f(\theta))-\theta\right ] \big/ \eta.
\end{equation}
%
% $$\hat{\Gamma}(f(\theta))=\lim_{\eta \rightarrow 0^+} \left [ \Gamma(\theta+\eta \cdot f(\theta))-\theta\right ] \big/ \eta.$$
%
Define
\begin{equation} \label{eqn:error_def}
    \epsilon_{\theta} = \frac{ \epsilon^J_{\theta} \left[ \kappa + H(d_{\theta}) \right] - J(\theta) \epsilon^H_{\theta} }{ \left[ \kappa + H(d_{\theta}) \right]^2}.
\end{equation}
%
Recall the ODE \eqref{eqn:actor_ode}
%
\begin{equation*}
\dot{\theta} = \hat{\Gamma} (\nabla \rho(\theta)), 
\end{equation*}
%
from \S\ref{sec:as_conv}, and consider the related ODE
%
\begin{equation} \label{eqn:biased_actor_ode}
\dot{\theta} = \hat{\Gamma} (\nabla \rho(\theta) + \epsilon_{\theta}). 
\end{equation}
%
Notice that, by the definition of $\hat{\Gamma}$, the right-hand side of \eqref{eqn:actor_ode} is simply $\Gamma(\nabla \rho(\theta))$ when there exists $\eta_0 > 0$ such that $\theta + \eta \nabla \rho(\theta) \in \Theta$, for all $\eta < \eta_0$. When such an $\eta_0$ does not exist, $\hat{\Gamma}(\nabla \rho(\theta))$ can be interpreted as the projected ODE $\dot{\theta} = \nabla \rho(\theta) + z(\theta)$, where $z(\theta)$ is the minimal force necessary to project $\theta$ back onto $\Theta$. Similar statements hold for \eqref{eqn:biased_actor_ode}. For further discussion of the definition of $\hat{\Gamma}$ and related results, see p.~191 of \cite{kushner1978stochastic}. For the projected ODE interpretation, see \S4.3 of \cite{kushner03}.
%
We now present the proof of Theorem \ref{thm:actor_conv}. We restate it here to ease the burden on the reader.

% \subsubsection{Proof of Theorem \ref{thm:actor_conv}} \label{sec:actor_conv_appendix}

\begin{customthm}{\ref{thm:actor_conv}}
%
%
	Let $\mathcal{Z}, \mathcal{Y}$ denote the sets of asymptotically stable equilibria of the ODEs \eqref{eqn:actor_ode}, \eqref{eqn:biased_actor_ode}, respectively. Given any $\varepsilon > 0$, define $\mathcal{Z}^{\varepsilon} = \{ z \ | \ \inf_{z' \in \mathcal{Z}} \| z - z' \| \leq \varepsilon \}$. For any $\theta \in \Theta$, let $\varepsilon_{\theta}$ be defined as in \eqref{eqn:error_def}. Under Assumptions \ref{assum:actor_conditions} and \ref{assum:stepsizes}, given any $\varepsilon > 0$, there exists $\delta > 0$ such that, for $\{ \theta_t \}$  obtained from the recursive scheme \eqref{eqn:irac_mu_j_update}-\eqref{eqn:irac_h_critic_update} and \eqref{eqn:irac_projected_policy_update}, if $\sup_t \| \epsilon_{\theta_t} \| < \delta$, then $\theta_t \to \mathcal{Z}^\varepsilon$ a.s. as $t \to \infty$.
\end{customthm}

% \begin{theorem}\label{thm:actor_conv}
% %
% %
% 	Let $\mathcal{Z}, \mathcal{Y}$ denote the sets of asymptotically stable equilibria of the ODEs \eqref{eqn:actor_ode}, \eqref{eqn:biased_actor_ode}, respectively. Given any $\varepsilon > 0$, define $\mathcal{Z}^{\varepsilon} = \{ z \ | \ \inf_{z' \in \mathcal{Z}} \| z - z' \| \leq \varepsilon \}$. For any $\theta \in \Theta$, let $\varepsilon_{\theta}$ be defined as in \eqref{eqn:error_def}. Under Assumptions \ref{assum:actor_conditions} and \ref{assum:stepsizes}, given any $\varepsilon > 0$, there exists $\delta > 0$ such that, for $\{ \theta_t \}$  obtained from the recursive scheme \eqref{eqn:irac_mu_j_update}-\eqref{eqn:irac_h_critic_update} and \eqref{eqn:irac_projected_policy_update}, if $\sup_t \| \epsilon_{\theta_t} \| < \delta$, then $\theta_t \to \mathcal{Z}^\varepsilon$ a.s. as $t \to \infty$.
% \end{theorem}

\begin{proof}
The main idea behind the proof is to show that the update scheme \eqref{eqn:irac_projected_policy_update} converges to a neighborhood of a stationary point by showing that it eventually tracks the ODE \eqref{eqn:actor_ode}. To do this, we first rewrite the update in \eqref{eqn:irac_projected_policy_update} as the sum of the true gradient direction and noise terms. We next argue that these noise terms are asymptotically negligible. We finally show that this noisy update scheme asymptotically tracks the biased ODE \eqref{eqn:biased_actor_ode}, which means that it converges to a neighborhood of the stationary points of \eqref{eqn:actor_ode}. The proof largely follows that of Thm.~1 in \cite{bhatnagar2009natural}, but with key modifications to accommodate complications arising from the fact that the objective to be minimized is a ratio; specifically, we ensure that: (i) the resulting noise terms are indeed asymptotically negligible, and (ii) the Lipschitz properties of the gradient $\nabla \rho(\theta)$ necessary for the ODE analysis are satisfied.
%

Let $\mathcal{F}_t = \sigma( \theta_k, k \leq t )$ denote the $\sigma$-algebra generated by the $\theta$-iterates up to time $t$.
%
%
Define
%
\begin{equation*}
    \delta_t = \frac {\delta^J_t \left[ \kappa + \mu^H_t \right] - \mu^J_t \delta^H_t}{\left[ \kappa + \mu^H_t \right]^2},
    \hspace{4mm}
    \delta^{\theta}_t = \frac{ \delta^{J, \theta}_t \left[ \kappa + H(d_{\theta}) \right] - J(\theta) \delta^{H, \theta}_t }{ \left[ \kappa + H(d_{\theta}) \right]^2}.
\end{equation*}
%
In addition, define the noise terms
%
\begin{align*}
    M^{(1)}_t &= \delta_t \nabla \log \pi_{\theta_t} (a_t | s_t) - \mathbb{E}_{\pi_{\theta_t}} \left[ \delta_t \nabla \log \pi_{\theta_t} (a_t | s_t) \ | \ \mathcal{F}_t \right], \\
    %
    &= \delta_t \nabla \log \pi_{\theta_t} (a_t | s_t) - \mathbb{E} \left[ \delta_t \nabla \log \pi_{\theta_t} (a_t | s_t) \ | \ \mathcal{F}_t \right], \\
    %
    M^{(2)}_t &= \mathbb{E}_{\pi_{\theta_t}} \left[ \left( \delta_t - \delta^{\theta_t}_t \right) \nabla \log \pi_{\theta_t} (a_t | s_t) \ | \ \mathcal{F}_t \right], \\
    %
    &= \mathbb{E} \left[ \left( \delta_t - \delta^{\theta_t}_t \right) \nabla \log \pi_{\theta_t} (a_t | s_t) \ | \ \mathcal{F}_t \right],
\end{align*}
%
as well as the function
%
\begin{align*}
    h(\theta_t) &= \mathbb{E}_{\pi_{\theta_t}} \left[ \delta^{\theta_t}_t \nabla \log \pi_{\theta_t} (a_t | s_t) \ | \ \mathcal{F}_t \right] \\
    %
    &= \mathbb{E}_{\pi_{\theta_t}} \left[ \delta^{\theta_t}_t \nabla \log \pi_{\theta_t} (a_t | s_t) \right],
\end{align*}
%
which is the gradient expression from Lemma \ref{lemma:bias_pg}. Note that simultaneously taking an expectation with respect to $\pi_{\theta_t}$ and conditioning on $\mathcal{F}_t$ is redundant, so we can suppress one or the other in our notation without altering the meaning. In what follows we will typically condition on $\mathcal{F}_t$ when we discussing the stochastic processes $\{ M^{(1)}_t \}, \{ M^{(2)}_t \}$, whereas we will take expectations with respect to $\pi_{\theta_t}$ when discussing the function~$h$.

We can now rewrite the projected actor update \eqref{eqn:irac_projected_policy_update} as
%
\begin{align*}
    \theta_{t+1} &= \Gamma \Big( \theta_t - \beta_t \delta_t \nabla \log \pi_{\theta_t} (a_t | s_t) \Big) \\
    %
    &= \Gamma \left( \theta_t - \beta_t \left[ h(\theta_t) + M^{(1)}_t + M^{(2)}_t \right] \right).
\end{align*}
%
We show that this update scheme asymptotically tracks the ODE \eqref{eqn:biased_actor_ode} a.s. by demonstrating that the noise terms $\{ M^{(1)}_t \}$ form an a.s. bounded martingale difference sequence, that the terms $\{ M^{(2)}_t \}$ are asymptotically negligible, and that $h$ is Lipschitz and thus the ODE is well-posed.

First notice that, since $\delta_t \rightarrow \delta^{\theta_t}_t$ a.s. by Lemma \ref{lemma:critics}, we have that $M^{(2)}_t \rightarrow 0$ a.s., so the noise terms $\{ M^{(2)}_t \}$ are indeed asymptotically negligible. Next, recall the tower property of conditional expectations, which states that, for any $\mathcal{F}$-measurable random variable $X$ and any sub-$\sigma$-algebras $\mathcal{G} \subset \mathcal{H} \subset \mathcal{F}$, we have $\mathbb{E} \left[ \mathbb{E} \left[ X | \mathcal{G} \right] | \mathcal{H} \right] = \mathbb{E} \left[ \mathbb{E} \left[ X | \mathcal{H} \right] | \mathcal{G} \right] = \mathbb{E} \left[ X | \mathcal{G} \right]$. Since $\mathcal{F}_t \subset \mathcal{F}_{t+1}$, for all $t \geq 0$, this implies that, for all $t \geq 0$,
%
\begin{align*}
    \mathbb{E} \left[ M^{(1)}_{t+1} | \mathcal{F}_t \right] &= \mathbb{E} \left[ \delta_{t+1} \nabla \log \pi_{\theta_{t+1}} (a_{t+1} | s_{t+1}) - \mathbb{E} \left[ \delta_{t+1} \nabla \log \pi_{\theta_{t+1}} (a_{t+1} | s_{t+1}) \ | \ \mathcal{F}_{t+1} \right] \ | \ \mathcal{F}_t \right] \\
    %
    &= \mathbb{E} \left[ \delta_{t+1} \nabla \log \pi_{\theta_{t+1}} (a_{t+1} | s_{t+1}) \ | \ \mathcal{F}_t \right] - \mathbb{E} \left[ \mathbb{E} \left[ \delta_{t+1} \nabla \log \pi_{\theta_{t+1}} (a_{t+1} | s_{t+1}) \ | \ \mathcal{F}_{t+1} \right] \ | \ \mathcal{F}_t  \right] \\
    %
    &= \mathbb{E} \left[ \delta_{t+1} \nabla \log \pi_{\theta_{t+1}} (a_{t+1} | s_{t+1}) \ | \ \mathcal{F}_t \right] - \mathbb{E} \left[ \delta_{t+1} \nabla \log \pi_{\theta_{t+1}} (a_{t+1} | s_{t+1}) \ | \ \mathcal{F}_t \right] \\
    %
    &= 0,
\end{align*}
%
so $\{ M^{(1)}_t \}$ is an $\mathcal{F}$-martingale difference sequence, where $\mathcal{F}$ is the filtration $\mathcal{F} = \{ \mathcal{F}_t \}$. To see that $M^{(1)}_t$ is a.s. bounded, first notice that $\mu^H_0 > 0$, and $0 < \inf_t d_{\theta_t}(s_t) \leq \sup_t d_{\theta_t}(s_t) \leq 1$, so by \eqref{eqn:irac_mu_h_update} $\{ \mu^H_t \}$ is uniformly bounded both above and below away from zero. A similar argument applies to $\{ \mu^J_t \}$, and, coupled with the a.s. boundedness of $\{ \omega^J_t \}$ and $\{ \omega^H_t \}$, this implies that $\{ \delta_t \}$ and thus $\{ M^{(1)}_t \}$ are a.s. bounded. As discussed in \S\S2.1-2.2 of \cite{borkar2008stochastic}, the facts that $\{ M^{(1)}_t \}$ is a.s. bounded martingale difference noise and $\{ M^{(2)}_t \}$ is asymptotically negligible ensure that, so long as the right-hand side of the ODE \eqref{eqn:biased_actor_ode} is Lipschitz, the iterates generated by \eqref{eqn:irac_projected_policy_update} will asymptotically track~it.

To see that $h$ is Lipschitz in $\theta$, first rewrite
%
\begin{align*}
    h(\theta_t) = \frac{1}{\left[ \kappa + H(d_{\theta_t}) \right]^2} \Big( & \left[ \kappa + H(d_{\theta_t}) \right] \mathbb{E}_{\pi_{\theta_t}} \left[ \delta^{J, \theta_t}_t \nabla \log \pi_{\theta_t} (a_t | s_t) \right] \\
    %
    &- J(\theta_t) \mathbb{E}_{\pi_{\theta_t}} \left[ \delta^{H, \theta_t}_t \nabla \log \pi_{\theta_t} (a_t | s_t) \right] \Big).
\end{align*}
%
We verify that each of the component terms in this expression is Lipschitz and bounded. Recall that a function is Lipschitz if it is continuously differentiable with bounded derivatives. 
First, as discussed in the proof of \cite{bhatnagar2009natural}, Lem.~5, $J(\theta)$, $d_{\theta}(s)$, $\nabla \pi_{\theta}(a | s)$, and $\Phi \omega^J_{\theta}$, are all Lipschitz and bounded, for all $s \in \mathcal{S}, a \in \mathcal{A}$. Together, these imply that the terms $J(\theta)$ and $\mathbb{E}_{\pi_{\theta}} \left[ \delta^{J, \theta}_t \nabla \log \pi_{\theta} (a_t | s_t) \right]$ are Lipschitz and bounded on $\Theta$. This means that the only remaining terms we need to inspect are $\kappa + H(d_{\theta})$, $1 / \left[ \kappa + H(d_{\theta}) \right]^2$, and $\mathbb{E}_{\pi_{\theta}} \left[ \delta^{H, \theta}_t \nabla \log \pi_{\theta} (a_t | s_t) \right]$.

Theorem \ref{thm:entropy_gradient} implies $\nabla H(d_{\theta})$ is continuous and bounded. To see this, notice that
%
\begin{align*}
    \nabla H(d_{\theta}) &= \mathbb{E}_{\pi_{\theta}} \Big[ \left( - \log d_{\theta}(s) - H(d_{\theta}) \right) \nabla \log \pi_{\theta}(a | s) \Big] \\
    %
    &= \sum_s d_{\theta}(s) \sum_a \pi_{\theta}(a | s) \Big[ \left( - \log d_{\theta}(s) - H(d_{\theta}) \right) \nabla \log \pi_{\theta}(a | s) \Big] \\
    %
    &= \sum_s d_{\theta}(s) \sum_a \nabla \pi_{\theta}(a | s) \Big[ \left( - \log d_{\theta}(s) - H(d_{\theta}) \right) \Big].
\end{align*}
%
By the ergodicity condition of Assumption \ref{assum:actor_conditions}, we have that $d_{\theta}(s) > 0$, for all $s \in \mathcal{S}$, which means that the $- \log d_{\theta}(s)$ is always defined. Since $d_{\theta}$ is continuous, we furthermore have that $- \log d_{\theta}(s)$ and $H(d_{\theta})$ are both continuous. The gradient $\nabla \pi_{\theta}(a | s)$ is continuous by Assumption \ref{assum:actor_conditions}. Finally, since $\Theta$ is a compact set, we know that $d_{\theta}(s), \nabla \pi_{\theta}(a | s), - \log d_{\theta}(s),$ and $H(d_{\theta})$ remain bounded, implying that $\nabla H(d_{\theta})$ is continuous and bounded, since it is formed by taking products and sums of continuous, bounded functions. $H(d_{\theta})$ is thus Lipschitz and bounded, as is the term $\kappa + H(d_{\theta})$, for any constant $\kappa \geq 0$. Furthermore, since $d_{\theta}(s) > 0$, for all $s \in \mathcal{S}$, and since $\Theta$ is compact, there exists some constant $B$ such that $\inf_{\theta \in \Theta} H(d_{\theta}) = B > 0$. This means that $1 / \left[ \kappa + H(d_{\theta}) \right]^2 \leq 1 / \left[ \kappa + B \right]^2$, for all $\theta \in \Theta$. The term $1 / \left[ \kappa + H(d_{\theta}) \right]^2$ is therefore Lipschitz and bounded, as well.

We now turn to the last remaining term. Notice that
%
\begin{align}
    \small
    \mathbb{E}_{\pi_{\theta}} & \left[ \delta^{H, \theta}_t \nabla \log \pi_{\theta} (a_t | s_t) \right] = \mathbb{E}_{\pi_{\theta}} \left[ \left( - \log d_{\theta}(s_t) - H(d_{\theta}) + \phi(s_{t+1})^{\top} \omega^H_{\theta} - \phi(s_t)^{\top} \omega^H_{\theta} \right) \nabla \log \pi_{\theta}(a_t | s_t) \right] \nonumber \\
    %
    &= \sum_s d_{\theta}(s) \sum_a \nabla \pi_{\theta}(a | s) \left[ - \log d_{\theta}(s) - H(d_{\theta}) - \phi(s)^{\top} \omega^H_{\theta}  + \sum_{s'} p(s' | s, a) \phi(s')^{\top} \omega^H_{\theta} \right]. \label{eqn:final_actor_term}
    \normalsize
\end{align}
%
As discussed above, $d_{\theta}(s), \pi_{\theta}(a | s), - \log d_{\theta}(s),$ and $H(d_{\theta})$ are all continuously differentiable with bounded derivatives on $\Theta$. Furthermore, given that $H(d_{\theta})$ is Lipschitz and bounded both above and away from zero, $\Phi \omega^H_{\theta}$ is Lipschitz and bounded for reasons analogous to those for $\Phi \omega^J_{\theta}$. Expression \eqref{eqn:final_actor_term} is thus Lipschitz and bounded. The function $h$ is thus Lipschitz as well, since it is formed by taking products and sums of Lipschitz, bounded functions.

The ODE \eqref{eqn:biased_actor_ode} is therefore well-posed, and its equilibrium set $\mathcal{Z}$ is well-defined. A similar argument to the one just presented can be used to show that \eqref{eqn:actor_ode} with equilibrium set $\mathcal{Y}$ is also well-posed. The remainder of the arguments in the proof of Lem.~5 in \cite{bhatnagar2009natural} now apply to prove that $\theta_t \rightarrow \mathcal{Y}$ a.s. as $t \rightarrow \infty$, and that, as $\sup_{\theta} \| \epsilon_{\theta} \| \rightarrow 0$, the trajectories of \eqref{eqn:biased_actor_ode} converge to those of \eqref{eqn:actor_ode}. In particular, this implies that, for a given $\varepsilon > 0$, there exists a $\delta > 0$ such that, if $\sup_{\theta} \| \epsilon_{\theta} \| < \delta$, then $\theta_t \rightarrow \mathcal{Z}^{\varepsilon}$ a.s. as $t \rightarrow \infty$.
%
\end{proof}

==> sections/Pseudocode.tex <==
\section{Entropy Maximization Algorithms} \label{sec:maxent_pseudocode}

\subsection{Maximizing $H(d_{\theta})$}

Algorithms for maximizing $H(d_{\theta})$ based on Theorem \ref{thm:entropy_gradient} are given below. These schemes can be easily combined with standard policy gradient algorithms to provide a state exploration bonus.

\vspace{1mm}


\begin{algorithm}[tb] % enter the algorithm environment
\caption{\texttt{MaxStateEntropyREINFORCE}} % give the algorithm a caption
\begin{algorithmic}[1] % enter the algorithmic environment
\STATE{{\textbf{Initialization:}} Select rollout length $K$, stepsizes $\eta < \tau$, parametrized policy class $\pi_{\theta}$. Randomly sample $\theta_0$; select $\widetilde{\mu}_0 > 0$; $t \gets 0$}
\REPEAT
    \STATE Generate trajectory $\{ (s_i, a_i) \}_{i = 1, \ldots, K}$ using policy $\pi_{\theta_t}$
    %
    \STATE Compute estimate $\widehat{d_{\theta_t}}(s)$, for each $s \in \mathcal{S}$ encountered
    %
    \STATE Compute estimate $\widehat{\mu^t(\theta_t)} = \frac{1}{K} \sum_{i=1}^K \left(- \log \widehat{d_{\theta_t}}(s_i) \right)$
    %
    \STATE Update $\widetilde{\mu}_t = (1 - \tau) \widetilde{\mu}_{t-1} + \tau \widehat{\mu^t(\theta_t)}$
    %
    \STATE Compute $\widehat{\nabla H(d_{\theta_t})} = \frac{1}{K} \sum_{i=1}^K \left[ - \log \widehat{d_{\theta_t}}(s_i) - \widetilde{\mu}_t \right] \nabla \log \pi_{\theta_t} ( a_i | s_i )$
    %
    \STATE $\theta_{t+1} = \theta_t + \eta \widehat{\nabla H(d_{\theta_t})}$
    %
    \STATE $t \gets t + 1$
\UNTIL{convergence}
\end{algorithmic}
%\end{minipage}
\end{algorithm}


\begin{algorithm}[tb] % enter the algorithm environment
\caption{\texttt{MaxStateEntropyActorCritic}} % give the algorithm a caption
\begin{algorithmic}[1] % enter the algorithmic environment
\STATE{{\textbf{Initialization:}} Select rollout length $K$, stepsizes $\tau$ and $\alpha < \beta$, parametrized policy class $\pi_{\theta}$, parametrized critic class $v_{\omega}$. Randomly sample $\theta_0, \omega_0$; select $\widetilde{\mu}_0 > 0$; $t \gets 0$.}
\REPEAT
    \STATE Generate trajectory $\{ (s_i, a_i) \}_{i = 1, \ldots, K}$ using policy $\pi_{\theta_t}$
    %
    \STATE Compute estimate $\widehat{d_{\theta_t}}(s)$, for each $s \in \mathcal{S}$ encountered
    %
    \STATE $\widehat{\mu^t(\theta_t)} = \frac{1}{K} \sum_{i=1}^K \left(- \log \widehat{d_{\theta_t}}(s_i) \right)$
    %
    \STATE $\widetilde{\mu}_t = (1 - \tau) \widetilde{\mu}_{t-1} + \tau \widehat{\mu^t(\theta_t)}$
    %
    \FOR{$i = 1, \ldots, K$}
        %
        % \STATE Compute TD error \\
        \STATE $\delta_i = - \log \widehat{d_{\theta_t}}(s_i) - \widetilde{\mu}_t + v_{\omega_t}(s_{i+1}) - v_{\omega_t}(s_i)$
        %
        \STATE where we stipulate $v_{\omega_t}(s_{K+1}) = 0$
    \ENDFOR
    %
    \STATE $\widehat{\nabla v_{\omega_t}} = \frac{1}{K} \sum_{i=1}^K \delta_i \nabla v_{\omega_t}(s_i)$
    %
    \STATE $\omega_{t+1} = \omega_t + \beta \widehat{\nabla v_{\omega_t}}$
    %
    \STATE $\widehat{\nabla H(d_{\theta_t})} = \frac{1}{K} \sum_{i=1}^K \delta_i \nabla \log \pi_{\theta_t} ( a_i | s_i )$
    %
    \STATE $\theta_{t+1} = \theta_t + \alpha \widehat{\nabla H(d_{\theta_t})}$ \\
    $t \gets t + 1$
\UNTIL{convergence}
\end{algorithmic}
%\end{minipage}
\end{algorithm}




\subsection{Maximizing $H(\lambda_{\theta})$}

Algorithms for maximizing $H(\lambda_{\theta})$ based on Corollary \ref{cor:state_action_entropy_gradient} are given next. Again, these schemes can be easily combined with standard policy gradient algorithms to provide a state-action exploration bonus. Note that, though we are estimating the entropy of the state-action occupancy measure, we only explicitly learn an approximation for the lower-dimensional state occupancy measure $d_{\theta}$.

\vspace{1mm}

\begin{algorithm}[tb] % enter the algorithm environment
\caption{\texttt{MaxStateActionEntropyREINFORCE}} % give the algorithm a caption
\begin{algorithmic}[1] % enter the algorithmic environment
\STATE{{\textbf{Initialization:}} Select rollout length $K$, stepsizes $\eta < \tau$, parametrized policy class $\pi_{\theta}$. Randomly sample $\theta_0$; select $\widetilde{\mu}_0 > 0$; $t \gets 0$}
\REPEAT
    \STATE Generate trajectory $\{ (s_i, a_i) \}_{i = 1, \ldots, K}$ using policy $\pi_{\theta_t}$
    %
    \STATE Compute estimate $\widehat{d_{\theta_t}}(s)$, for each $s \in \mathcal{S}$ encountered
    %
    \STATE Compute estimate $\widehat{\mu^t(\theta_t)} = \frac{1}{K} \sum_{i=1}^K \left(- \log \widehat{d_{\theta_t}}(s_i) - \log \pi_{\theta_t}(a_i | s_i) \right)$
    %
    \STATE Update $\widetilde{\mu}_t = (1 - \tau) \widetilde{\mu}_{t-1} + \tau \widehat{\mu^t(\theta_t)}$
    %
    \STATE Compute $\widehat{\nabla H(\lambda_{\theta_t})} = \frac{1}{K} \sum_{i=1}^K \left[ - \log \widehat{d_{\theta_t}}(s_i) - \log \pi_{\theta_t}(a_i | s_i) - \widetilde{\mu}_t \right] \nabla \log \pi_{\theta_t} ( a_i | s_i )$
    %
    \STATE $\theta_{t+1} = \theta_t + \eta \widehat{\nabla H(\lambda_{\theta_t})}$
    %
    \STATE $t \gets t + 1$
\UNTIL{convergence}
\end{algorithmic}
%\end{minipage}
\end{algorithm}


\begin{algorithm}[tb] % enter the algorithm environment
\caption{\texttt{MaxStateActionEntropyActorCritic}} % give the algorithm a caption
\begin{algorithmic}[1] % enter the algorithmic environment
\STATE{{\textbf{Initialization:}} Select rollout length $K$, stepsizes $\tau$ and $\alpha < \beta$, parametrized policy class $\pi_{\theta}$, parametrized critic class $v_{\omega}$. Randomly sample $\theta_0, \omega_0$; select $\widetilde{\mu}_0 > 0$; $t \gets 0$.}
\REPEAT
    \STATE Generate trajectory $\{ (s_i, a_i) \}_{i = 1, \ldots, K}$ using policy $\pi_{\theta_t}$
    %
    \STATE Compute estimate $\widehat{d_{\theta_t}}(s)$, for each $s \in \mathcal{S}$ encountered
    %
    \STATE $\widehat{\mu^t(\theta_t)} = \frac{1}{K} \sum_{i=1}^K \left(- \log \widehat{d_{\theta_t}}(s_i) - \log \pi_{\theta_t}(a_i | s_i) \right)$
    %
    \STATE $\widetilde{\mu}_t = (1 - \tau) \widetilde{\mu}_{t-1} + \tau \widehat{\mu^t(\theta_t)}$
    %
    \FOR{$i = 1, \ldots, K$}
        %
        \STATE $\delta_i = - \log \widehat{d_{\theta_t}}(s_i) - \log \pi_{\theta_t}(a_i | s_i) - \widetilde{\mu}_t + v_{\omega_t}(s_{i+1}) - v_{\omega_t}(s_i)$
        %
        \STATE here we stipulate $v_{\omega_t}(s_{K+1}) = 0$
    \ENDFOR
    %
    \STATE $\widehat{\nabla v_{\omega_t}} = \frac{1}{K} \sum_{i=1}^K \delta_i \nabla v_{\omega_t}(s_i)$
    %
    \STATE $\omega_{t+1} = \omega_t + \beta \widehat{\nabla v_{\omega_t}}$
    %
    \STATE $\widehat{\nabla H(\lambda_{\theta_t})} = \frac{1}{K} \sum_{i=1}^K \delta_i \nabla \log \pi_{\theta_t} ( a_i | s_i )$
    %
    \STATE $\theta_{t+1} = \theta_t + \alpha \widehat{\nabla H(\lambda_{\theta_t})}$
    %
    \STATE $t \gets t + 1$
\UNTIL{convergence}
\end{algorithmic}
%\end{minipage}
\end{algorithm}


\newpage

\section{Pseudocode for \texttt{VanillaActorCritic}} \label{sec:vanillaac_pseudocode}


\begin{algorithm}[tb] % enter the algorithm environment
\caption{\texttt{VanillaActorCritic}} \label{alg:vanilla_ac} % give the algorithm a caption
\begin{algorithmic}[1] % enter the algorithmic environment
\STATE{{\textbf{Initialization:}} Select rollout length $K$, stepsizes $\tau$ and $\alpha < \beta$, parametrized policy class $\pi_{\theta}$, parametrized critic class $v_{\omega}$. Randomly sample $\theta_0, \omega_0$; select $\widetilde{\mu}_0 > 0$; $t \gets 0$.}
\REPEAT
    \STATE Generate trajectory $\{ (s_i, a_i) \}_{i = 1, \ldots, K}$ using policy $\pi_{\theta_t}$
    %
    \STATE $\widehat{J(\theta_t)} = \frac{1}{K} \sum_{i=1}^{K} c(s_i, a_i)$
    %
    \STATE $\widetilde{\mu}_t = (1 - \tau) \widetilde{\mu}_{t-1} + \tau \widehat{J(\theta_t)}$
    %
    \FOR{$i = 1, \ldots, K$}
        %
        \STATE $\delta_i = c(s_i, a_i) - \widetilde{\mu}_t + v_{\omega_t}(s_{i+1}) - v_{\omega_t}(s_i)$
        %
        \STATE where we stipulate $v_{\omega_t}(s_{K+1}) = 0$
    \ENDFOR
    %
    \STATE $\widehat{\nabla v_{\omega_t}} = \frac{1}{K} \sum_{i=1}^K \delta_i \nabla v_{\omega_t}(s_i)$
    %
    \STATE $\omega_{t+1} = \omega_t + \beta \widehat{\nabla v_{\omega_t}}$
    %
    \STATE $\widehat{\nabla J(\theta_t)} = \frac{1}{K} \sum_{i=1}^K \delta_i \nabla \log \pi_{\theta_t}(a_i | s_i)$
    %
    \STATE $\theta_{t+1} = \theta_t - \alpha \widehat{\nabla J(\theta_t)}$
    %
    \STATE $t \gets t + 1$
\UNTIL{convergence}
\end{algorithmic}
%\end{minipage}
\end{algorithm}


For completeness, we provide pseudocode in Algorithm \ref{alg:vanilla_ac} for the version of average-cost actor-critic that we compared against in our experimental results.

==> sections/Related_Works.tex <==
\section{Related Work} \label{sec:related_work}

A large number of previous works have incorporated information-theoretic tools and related exploration-encouraging methods into sequential decision-making problems in an effort to tackle the exploration/exploitation trade-off. In this section we provide a literature review of related efforts for the multi-armed bandit (MAB) and reinforcement learning (RL) settings.
%
\\ \\
\noindent \textbf{Multi-Armed Bandits.} In the MAB setting, classic approaches include Gittins index methods, upper confidence bound (UCB) methods, Thompson sampling (TS), and information-directed sampling (IDS). Viewing the MAB as a certain class of optimal stopping problem, it was first shown in \cite{gittins1979bandit} how to obtain an optimal policy via computation of the Gittins index. Though Gittins index-based methods are theoretically guaranteed to provide optimal policies, computational methods based on them, such as that outlined in \S35.5 of \cite{lattimore2020bandit}, rely on knowledge or a learned model of the system dynamics, making them impractical for complex problems. UCB methods \cite{abbasi2011improved, bubeck2011x, srinivas2012information} use an optimistic over-estimate of action rewards coupled with greedy policies to encourage exploration of infrequently chosen actions. TS schemes \cite{agrawal2012analysis}, on the other hand, iteratively update the agent's belief about the identity of the optimal action based on experience, all while choosing actions as if the current belief is optimal. Interestingly for our setting, \cite{russo2016information} uses an information ratio for MABs, defined in equation \eqref{eqn:MAB_info_ratio} below, as an analysis tool to prove that TS leads to superior regret bounds. A work related to \cite{russo2016information}, \cite{russo2014learning} develops the IDS scheme to balance regret with information acquisition by explicitly minimizing the MAB information ratio at each timestep, leading to better bounds than both TS and UCB in many cases. However, it is often unclear how to use the information ratio in MAB settings to devise new algorithms.
\\ \\
\noindent \textbf{Information in Reinforcement Learning.} Moving to the MDP setting, a vast literature has grown up around methods for balancing exploration and exploitation. Within this literature, many works leverage information-theoretic connections to encourage exploration of the state and action spaces. An early connection between policy gradient methods and information-theoretic techniques is the introduction of Fischer information-based preconditioners for gradient updates in the natural policy gradient method \cite{amari1998natural, kakade2001natural}, which improves gradient updates by taking the information geometry of the policy parameterization into account. More recently, policy entropy regularization, where a bonus is provided for policies that behave more randomly\footnote{Policy entropy is defined as $H(\pi(\cdot | s)) = - \sum_a \pi(a | s) \log \pi(a | s)$. When used as a regularizer, larger values of $H(\pi(\cdot | s))$ are encouraged.}, has seen both great practical success \cite{haarnoja2018soft} and leads to policies that inherit favorable theoretical attributes of proximal point methods \cite{mei2020global}. Similar to the MAB setting, UCB-type exploration bonuses have also been successfully used to encourage exploration in the RL setting. In particular, certain forms of UCB-induced exploration lead to regret bounds that are comparable to model-based methods when used in conjunction with the model-free Q-learning algorithm in the tabular case \cite{jin2018q}. In a distinct, but related direction, the recent work \cite{furuta2021policy} proposes a novel, information-theoretic measure of task complexity, called policy(-optimal) information capacity, and empirically demonstrates how it can be used to determine the difficulty of a range of common RL problems.
\\ \\
\noindent \textbf{Maximum Entropy Exploration.} In recent years RL for maximum entropy exploration has seen increasing interest. Unlike the \textit{policy} entropy regularization described above, the schemes developed in \cite{hazan2019provably, zhang2020variational} provide a way to directly maximize the entropy $H(d_{\theta})$ of the state occupancy measure $d_{\theta}$. In the absence of a reward signal, \cite{hazan2019provably} argue that it is reasonable for an agent to instead maximize some measure of coverage of the state space, such as $H(d_{\theta})$. The authors develop a novel algorithm for maximizing a concave reward functional of the state occupancy measure (which includes entropy), and, given access to suitable oracles, they prove convergence to a nearly optimal policy and provide sample complexity bounds. Similar to \cite{hazan2019provably}, the variational policy gradient algorithm proposed in \cite{zhang2020variational} studies the problem of optimizing reward functionals that are not as nicely behaved as the standard discounted reward. The saddle-point algorithm that they develop can be applied to maximize any objective that can be formulated as a concave function of the state-action occupancy measure. Furthermore, it is shown by introducing the notion of \textit{hidden concavity} that, when viewed as an optimization problem over the parameter space, the problem has no spurious local extrema, i.e. every stationary point is global optimal. This notion of hidden concavity is important for our current work, as we generalize it to prove a similar result for our algorithms. Though it does not explicitly consider entropy maximization, the recent work \cite{zhang2021beyond} explores a new class of risk-sensitive RL methods by considering optimization over the space of state-action occupancy measures. This is closely related to both \cite{zhang2020variational} and our current paper, since in all three the dual of the primal linear programming formulation of the underlying MDP is modified to incorporate new learning objectives: exploration in \cite{zhang2020variational} and the present work, and risk-sensitivity in \cite{zhang2021beyond}.
\\ \\
\noindent \textbf{Information Ratios.} Of all the related works described in this section, the work \cite{russo2014learning} on IDS for MABs discussed above and the recent work \cite{lu2021reinforcement} developing an information ratio for general problems are most relevant to our current paper. In \cite{lu2021reinforcement}, the authors develop a powerful, abstract framework for reasoning about the design of algorithms for solving sequential decision-making problems, including MDPs. They generalize the MAB information ratio of \cite{russo2014learning} to this setting, resulting in the $\tau$-information ratio defined in equation \eqref{eqn:general_info_ratio} below, and regret bounds and algorithmic schemes are provided.
In the IDS scheme proposed in \cite{russo2014learning}, the information ratio is minimized at each step to obtain an action-selection distribution that balances minimizing regret with gaining information about the optimal action. One of the goals of \cite{lu2021reinforcement} is to use the $\tau$-information ratio to develop similar sampling schemes for the RL setting to guide action selection at each step. Due to inherent difficulties in minimizing regret and estimating mutual information, the authors acknowledge that optimizing their information ratio directly is typically intractable. For this reason they develop a series of useful surrogate or \textit{pseudo}-information ratios to optimize instead, resulting in the value-IDS and variance-IDS schemes. Variance-IDS, the more computationally tractable of the two, requires maintaining and updating belief distributions over the set of possible action-value functions as well as solving a convex optimization problem over the action set %$\mc{D}(\mc{A})$ 
at each step. This restricts its applicability to smaller problems and makes it difficult to scale to continuous action spaces. The use of epistemic neural networks to overcome the problem of maintaining belief distributions is explored, however, and promising empirical results are provided demonstrating performance comparable to or better than TS on problems where information acquisition is~key.
